A high order conservative semi-Lagrangian discontinuous Galerkin method for two-dimensional transport simulations

In this paper, we develop a class of high order conservative semi-Lagrangian (SL) discontinuous Galerkin (DG) methods for solving multi-dimensional linear transport equations. The methods rely on a characteristic Galerkin weak formulation, leading to $L^2$ stable discretizations for linear problems. Unlike many existing SL methods, the high order accuracy and mass conservation of the proposed methods are realized in a non-splitting manner. Thus, the detrimental splitting error, which is known to significantly contaminate long term transport simulations, will be not incurred. One key ingredient in the scheme formulation, borrowed from CSLAM [Lauritzen, Nair, and Ullrich, 2010], is the use of Green's theorem which allows us to convert volume integrals into a set of line integrals. The resulting line integrals are much easier to approximate with high order accuracy, hence facilitating the implementation. Another novel ingredient is the construction of quadratic curves in approximating sides of upstream cell, leading to quadratic-curved quadrilateral upstream cells. Formal third order accuracy is obtained by such a construction. The desired positivity-preserving property is further attained by incorporating a high order bound-preserving filter. To assess the performance of the proposed methods, we test and compare the numerical schemes with a variety of configurations for solving several benchmark transport problems with both smooth and nonsmooth solutions. The efficiency and efficacy are numerically verified.

==> analysis.tex <==
\section{Theoretical Analysis}
	In this section, we rigorously establish the $L^2$ stability of the proposed scheme for the $P^1$ case in two dimensions. For illustrative purposes, we introduce the following notations: Denote $\bx = (x,y)$, and $\bX(t)=(X_1(t),X_2(t)) = \bX(t;\bx,t_0)$ that solves the characteristics equation
	\begin{equation}
	\label{eq:charact}
	\left\{
	\begin{array}{l}
	\displaystyle\frac{d \bX(t)}{dt} = \ba(\bX(t),t)\\[2mm]
	\bX(t_0) = \bx,
	\end{array}	
	\right.
	\end{equation}
	with $\ba=(a,b)$ being the velocity field.
\subsection{$L^2$ Stability Analysis}

\begin{lem}\label{lem:1}
	Assume that the coefficient $a(\bx, t)\in C^0(C^2(\Omega);[0,T])$, $\bX(t)$ solves the initial valve problem \eqref{eq:charact}.
%\begin{equation}
%\left\{
%\begin{array}{l}
%\displaystyle\frac{d \bX(t)}{dt} = \ba(\bX(t),t)\\[2mm]
%\bX(t_0) = \bx,
%\end{array}	
%\right.
%\end{equation}
%where $\bx=(x,y)$, $\bX(t)=\bX(t;\bx,t):=(x(t;x, t_0),y(t;y, t_0))$, and  $\ba=(a(\bX(t),t),b(\bX(t),t))$.
Let $\bY=\frac{\partial\bX}{\partial\bx}$ and $\bZ = \frac{\partial\bY}{\partial\bx}$, then
$$|\bY| \le e^{C_0(t-t_0)}\quad  |\bZ| \le e^{2C_0(t-t_0)}-e^{C_0(t-t_0)},$$
where $C_0=\max_{0\le t\le T}\|a(\bx,t)\|_{C^2(\Omega)}$.
\end{lem}
Proof: The proof follows the standard argument of the differentiability of the solution with the initial conditions.

\begin{thm}
	Assume that the coefficient $a(\bx, t)\in C^0(C^2(\Omega);[0,T])$, the characteristics are exactly tracked in the algorithm and the ratio CFL:=$\Delta t/h$ is any fixed positive number which can be arbitrarily large, then the scheme with approximation space $\mathcal{G}_h^1$ is $L^2$ stable when the mesh is sufficiently refined.
\end{thm}
Proof: We start with the weak formulation \eqref{2d_temporal} and let the test function $\Psi(\bx)$ be $u^{n+1}$ with $\bx = (x,y)$, then we get
\begin{equation}
\label{eq:stability}
\int_{A_j} \left(u^{n+1}(\bx)\right)^2 d\bx = \int_{A_j^\star}u^{n}(\bx)\left(\bP^1 u^{n+1}\left(\bX(t^{n+1})\right)\right) d\bx,
\end{equation}
where $\bP^1$ is the projection operator defined in Subsection \ref{sec:p1} and $\bX(t)$ solves the initial value problem
\begin{equation}
\label{eq:ivp}
\left\{
\begin{array}{l}
	\displaystyle\frac{d \bX(t)}{dt} = 
	\ba(\bX(t),t)\\[2mm]
	\bX(t^{n}) = \bx.
	\end{array}	
	\right.
\end{equation}
A direct application of the Cauchy-Schwarz inequality to \eqref{eq:stability} yields 
\begin{equation}
\|u^{n+1}(\bx)\|^2_{L^2(A_j)}=\|u^n(\bx)\|_{L^2(A_j)}\|\bP^1 u^{n+1}\left(\bX(t^{n+1})\right)\|_{L^2(A_j^\star)}.
\end{equation}
%
We further write
\begin{equation*}
\bP^1 u^{n+1}(\bX(t^{n+1})) = u^{n+1}(\bX(t^{n+1})) - (u^{n+1}(\bX(t^{n+1}))-\bP^1 u^{n+1}(\bX(t^{n+1}))),
\end{equation*}
and hence
\begin{equation}
\label{eq:proj1}
\|\bP^1 u^{n+1}(\bX(t^{n+1}))\|_{L^2(A_j^\star)} \leq \|u^{n+1}(\bX(t^{n+1}))\|_{L^2(A_j^\star)} + \|(u^{n+1}(\bX(t^{n+1}))-\bP^1 u^{n+1}(\bX(t^{n+1})))\|_{L^2(A_j^\star)}.
\end{equation}
We consider the second term first.
Note that $u^{n+1}(\bX(t))$ is a $P^1$ polynomial with respect to $\bX(t)$. In addition, $\bX(t)$ solves \eqref{eq:ivp} and hence is twice continuously differentiable with respect to  $\bx$ thanks to $a(\bx,t)\in  C^0(C^2(\Omega),[0,T])$. Therefore, $u^{n+1}(\bX(t^{n+1}))\in H^2(A^\star)$, and we have the following estimate
\begin{equation}
\label{eq:interpolation}
\|u^{n+1}(\bX(t^{n}))-\bP^1 u^{n+1}(\bX(t^{n}))\|_{L^2(A_j^\star)}\leq C_0 h^2|u^{n+1}(\bX(t^{n}))|_{H^2(A_j^\star)},
\end{equation}
where $C_0$ depends on the shape of $A_j^\star$, in particular, the ratio
$\sigma = \frac{d_{A^\star_j}}{\rho_{A^\star_j}}$ with
$$d_{A^\star_i}=\text{diameter of }A_j^\star \quad \text{and} \quad \rho_{A^\star_j} =\sup\{\text{diameter of } B|\, B \text{ is a ball contains in }A^\star_j\}.$$
\textcolor{red}{Under the assumption that  CFL$=\Delta t/h$ is a fixed number, and $a\in C^0(C^2(\Omega);[0,T])$, then if the mesh is sufficiently refined, equivalently  $h$ and $\Delta t$ are small enough, we have $\sigma$ is uniformly  bounded. In other words, we require that the spatial mesh size $h$ and the time step $\Delta t$ should be able resolve the deformation of the mesh over one time step, even though  CFL can be arbitrarily large.}


Now, we estimate $|u^{n+1}(\bX(t^{n+1}))|_{H^2(A^\star)}$. By the chain rule, we have
\begin{equation}
\frac{\partial u^{n+1}}{\partial x}=\frac{\partial u^{n+1}}{\partial X_1}\frac{\partial X_1}{\partial x}+\frac{\partial u^{n+1}}{\partial X_2}\frac{\partial X_2}{\partial x}.
\end{equation}
Furthermore, since $u^{n+1}$ is a $P^1$ polynomial with $\bX$, then $\frac{\partial u^{n+1}}{\partial X_1}$ and $\frac{\partial u^{n+1}}{\partial X_2}$ are both constant. Therefore
\begin{equation}
 %\quad
%\frac{\partial u^{n+1}}{\partial y}=\frac{\partial u^{n+1}}{\partial \bX_1}\frac{\partial \bX_1}{\partial y}+\frac{\partial u^{n+1}}{\partial \bX_1}\frac{\partial \bX_1}{\partial y},
\frac{\partial^2 u^{n+1}}{\partial x^2}=\frac{\partial u^{n+1}}{\partial X_1}\frac{\partial^2 X_1}{\partial x^2}+\frac{\partial u^{n+1}}{\partial X_2}\frac{\partial^2 X_2}{\partial x^2}.
\end{equation}
Similarly,
\begin{align}
%\quad
%\frac{\partial u^{n+1}}{\partial y}=\frac{\partial u^{n+1}}{\partial \bX_1}\frac{\partial \bX_1}{\partial y}+\frac{\partial u^{n+1}}{\partial \bX_1}\frac{\partial \bX_1}{\partial y},
\frac{\partial^2 u^{n+1}}{\partial x\partial y}&=\frac{\partial u^{n+1}}{\partial X_1}\frac{\partial^2 X_1}{\partial x^2}+\frac{\partial u^{n+1}}{\partial X_2}\frac{\partial^2 X_2}{\partial x\partial y},\\
\frac{\partial^2 u^{n+1}}{\partial y^2}&=\frac{\partial u^{n+1}}{\partial X_1}\frac{\partial^2 X_1}{\partial y^2}+\frac{\partial u^{n+1}}{\partial X_2}\frac{\partial^2 X_2}{\partial y^2}.
\end{align}
Hence,
\begin{equation}
|u^{n+1}(\bX(t^{n+1}))|_{H^2(A^\star_j)}\leq |\nabla_\bX u^{n+1}|_{L^2(A^\star_j)}|\bZ|_{L^\infty(A^\star_j)},
\end{equation}
where $\bZ = \frac{\partial^2 \bX}{\partial \bx^2}.$
Combining this with lemma \ref{lem:1}, we further obtain
\begin{equation}
\label{eq:h2}
|u^{n+1}(\bX(t^{n+1}))|_{H^2(A^\star_j)}\leq C_2|\nabla_\bX u^{n+1}|_{L^2(A^\star_j)},
\end{equation}
where $C_2 = e^{C\Delta t}(e^{C\Delta t}-1)$.
Now we estimate the right hand side of \eqref{eq:h2}. Following the characteristics forward for $t^n$ to $t^{n+1}$, we have
\begin{equation}
\label{eq:diff_area}
|\nabla_\bX u^{n+1}(\bX(t^{n+1}))|_{L^2(A^\star_j)}=|\nabla_\bx u^{n+1}(\bx)|_{L^2(A^{\star\star}_j)},
\end{equation}
where $A^{\star\star}_j$ is the upstream cell of $A^{\star}_j$ at $t=t^{n+1}$, see Figure \ref{schematic:analysis} (a). Further note that $A^{\star\star}_j$ in general does not coincide with $A_j$, except the four vertices, and hence we in fact consider $u^{n+1}(\bx)$ as the extension from $A_j$ to $A_j^{\star\star}$ in \eqref{eq:diff_area}.

\textcolor{red}{We again require that $h$ and $\Delta t$ are sufficiently small such that the boundary of $A^{\star\star}_i$ only deviates the boundary of $A_i$ by $C_2h^2$, where $C_2$ depends on $C$, CFL and $\Delta t$. And it can be attained due to Lemma 1.} As such, the difference in area between $A_j$ and $A_j^{\star\star}$ is of the order $h^3$. Since the gradient $\nabla_\bx u^{n+1}$ is a constant vector, we have
\begin{equation}
\label{eq:grad}
|\nabla_\bx u^{n+1}|_{L^2(A^{\star\star}_i)}\leq (1+C_3 h^3)|\nabla_\bx u^{n+1}|_{L^2(A_i)}\leq C_4h^{-1}\|u^{n+1}\|_{L^2(A_i)},
\end{equation}
due to the inverse inequality. Combining the estimates \eqref{eq:interpolation}, \eqref{eq:h2}, and \eqref{eq:grad} yields
\begin{equation}
\label{eq:e2}
\|u^{n+1}(\bX(t^{n+1}))-\bP^1 u^{n+1}(\bX(t^{n+1}))\|_{L^2(A_j^\star)}\leq C_1^\star h\|u^{n+1}\|_{L^2(A_j)}.
\end{equation}


 Lastly, we consider the first term in \eqref{eq:proj1}. As in \eqref{eq:diff_area}, we have
\begin{equation}
\|u^{n+1}(\bX(t^{n+1}))\|_{L^2(A^\star_j)}=\|u^{n+1}(\bx)\|_{L^2(A^{\star\star}_j)}.
\end{equation}
Note that $u^{n+1}(\bx)$ is a linear function on $A_i^{\star\star}$. By the trace inequality and the inverse inequality (add detail when a figure is added), we are able to obtain
\begin{equation}
\label{eq：e1}
\|u^{n+1}(\bX(t^{n}))\|_{L^2(A^\star_j)}\leq (1+C_2^\star h)\|u^{n+1}(\bx)\|_{L^2(A_j)}.
\end{equation}

Combining \eqref{eq:stability}, \eqref{eq:proj1}, \eqref{eq:e1} and \eqref{eq:e2}, we arrive
\begin{equation}
\|u^{n+1}(\bx)\|_{L^2(A_j)}\leq (1+C^\star h) \|u^n(\bx)\|_{L^2(A^\star_j)}.
\end{equation}
Summing over $j$ and further noting that $h = \Delta t/$CFL, we obtain
\begin{align}
\|u^{n+1}(\bx)\|_{L^2(\Omega)}&\leq (1+C\Delta t)^{n+1} \|u^0(\bx)\|_{L^2(\Omega)}\\
&\leq e^{CT}\|u^0(\bx)\|_{L^2(\Omega)},
\end{align}
where $C=C^{\star}/$CFL and the final time $T=(n+1)\Delta t$.

\begin{rem}
    For the sake of stability, we do not set any restriction on the CFL number, but require  that $h$ and $\Delta t$ are able to resolve the deformed mesh when following the characteristics one time step backward or forward. Otherwise, the scheme may be  unstable. A similar phenomenon is observed for the Eulerian DG methods on a curved domain, which is known unstable when the mesh is not sufficiently refined or the geometry of the boundary is under-resolved, see \cite{zhang2016curved}.
\end{rem}



\begin{figure}[h]
\centering
\subfigure[]{
\begin{tikzpicture}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%mesh
    \draw[black,thin] (0,0.5) node[left] {} -- (5.5,0.5)
                                        node[right]{};
    \draw[black,thin] (0,2.) node[left] {$$} -- (5.5,2)
                                        node[right]{};
    \draw[black,thin] (0,3.5) node[left] {$$} -- (5.5,3.5)
                                        node[right]{};
    \draw[black,thin] (0,5 ) node[left] {$$} -- (5.5,5)
                                        node[right]{};
                                        %%%%%%%%%%%
    \draw[black,thin] (0.5,0) node[left] {} -- (0.5,5.5)
                                        node[right]{};
    \draw[black,thin] (2,0) node[left] {$$} -- (2,5.5)
                                        node[right]{};
    \draw[black,thin] (3.5,0) node[left] {$$} -- (3.5,5.5)
                                        node[right]{};
    \draw[black,thin] (5,0) node[left] {$$} -- (5,5.5)
                                        node[right]{};
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% background element
    \fill [blue] (3.5,3.5) circle (2pt) node[] {};
    \fill [blue] (5,3.5) circle (2pt) node[] {};
    \fill [blue] (3.5,5) circle (2pt) node[below right] {} node[above left] {};
    \fill [blue] (5,5) circle (2pt) node[] {};

     \draw[thick,blue] (3.5,3.5) node[left] {} -- (3.5,5)
                                        node[right]{};
      \draw[thick,blue] (3.5,3.5) node[left] {} -- (5,3.5)
                                        node[right]{};
       \draw[thick,blue] (3.5,5) node[left] {} -- (5,5)
                                        node[right]{};
        \draw[thick,blue] (5,3.5) node[left] {} -- (5,5)
                                        node[right]{};
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Lagrangian element
    \fill [red] (1.,1) circle (2pt) node[above right,black] {};
    \fill [red] (3,1) circle (2pt) node[] {};
    \fill [red] (1,2.5) circle (2pt) node[below right] {$A_j^\star$} node[above left] {};
    \fill [red] (2.5,2.5) circle (2pt) node[] {};

     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%A **

            \draw [brown, very thick] (3.5,3.5)node[right,scale=1.0]{}
        to[out=50,in=230] (3.5,5) node[] {};
        
        \draw [brown,very thick] (3.5,3.5)node[right,scale=1.0]{}
        to[out=340,in=200] (5,3.5) node[] {};
        
        \draw [brown,very thick] (3.5,5)node[right,scale=1.0]{}
        to[out=340,in=200] (5,5) node[] {};
        
        \draw [brown,very thick] (5,3.5)node[right,scale=1.0]{}
        to[out=70,in=290] (5,5) node[] {};
        
        \node [below right,brown] at (3.5,5) {$A_j^{\star\star}$};
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

     \draw[-latex,dashed] (1,2.50) node[right,scale=1.0]{}
        to[out=70,in=240] (3.5,5)node[] {};

     \draw (0.5+0.01,2-0.01) node[fill=white,below right] {};


    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \draw [thick,red] (1,1)-- (3,1) node[] {};
 \draw [thick,red] (1,2.5) -- (1,1) node[] {};
        \draw [thick,red] (1,2.5)--(2.5,2.5) node[] {};
        \draw [thick,red] (3,1)--(2.5,2.5) node[] {};
   
        
\end{tikzpicture}
}
\subfigure[]{

\begin{tikzpicture}[scale = 2]
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%mesh
  
    \draw[black,thin] (3,3.5) node[left] {$$} -- (5.5,3.5)
                                        node[right]{};
    \draw[black,thin] (3,5 ) node[left] {$$} -- (5.5,5)
                                        node[right]{};
                                        %%%%%%%%%%%

    \draw[black,thin] (3.5,3) node[left] {$$} -- (3.5,5.5)
                                        node[right]{};
    \draw[black,thin] (5,3) node[left] {$$} -- (5,5.5)
                                        node[right]{};
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% background element
    \fill [blue] (3.5,3.5) circle (2pt) node[] {};
    \fill [blue] (5,3.5) circle (2pt) node[] {};
    \fill [blue] (3.5,5) circle (2pt) node[below right] {} node[above left] {};
    \fill [blue] (5,5) circle (2pt) node[] {};

     \draw[thick,blue] (3.5,3.5) node[left] {} -- (3.5,5)
                                        node[right]{};
      \draw[thick,blue] (3.5,3.5) node[left] {} -- (5,3.5)
                                        node[right]{};
       \draw[thick,blue] (3.5,5) node[left] {} -- (5,5)
                                        node[right]{};
        \draw[thick,blue] (5,3.5) node[left] {} -- (5,5)
                                        node[right]{};
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%A **

            \draw [brown, very thick] (3.5,3.5)node[right,scale=1.0]{}
        to[out=50,in=230] (3.5,5) node[] {};

        \draw [brown,very thick] (3.5,3.5)node[right,scale=1.0]{}
        to[out=340,in=200] (5,3.5) node[] {};

        \draw [brown,very thick] (3.5,5)node[right,scale=1.0]{}
        to[out=340,in=200] (5,5) node[] {};

        \draw [brown,very thick] (5,3.5)node[right,scale=1.0]{}
        to[out=70,in=290] (5,5) node[] {};

        \node [below right=2pt,brown] at (3.5,5) {$A_j^{\star\star}$};
        
        \node [below=8pt] at (4.25,3.5) {$g(x)$};
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
        
\end{tikzpicture}

}
\caption{}
\label{schematic:analysis}
\end{figure}

\subsection{Error Estimate}


==> append.tex <==
\section{Appendix}
\subsection{Fifth-order Runge-Kutta method}
\label{RK5}
A fifth-order Runge-Kutta method in \cite{butcher2008numerical},
  \begin{equation}
  x(t_n) \approx x(t_{n+1}) - \frac{1}{90} ( 7k_1 + 32k_3+12k_4+32k_5+7k_6 )\Delta t,
  \end{equation}
  where
    \begin{equation*}
  \begin{split}
  &k_1 = a( x(t_{n+1} ),t_{n+1}  ) ,\\
  &k_2 = a( x(t_{n+1} )-\frac14k_1\Delta t ,t_{n+1} -\frac14 \Delta t  ) ,\\
  &k_3 = a( x(t_{n+1} )-\frac18k_1\Delta t-\frac18k_2\Delta t, t_{n+1}-\frac14\Delta t ),\\
  &k_4 = a( x(t_{n+1} )+\frac12k_2\Delta t-k_3\Delta t, t_{n+1} -\frac12\Delta t  ),\\
  &k_5 = a( x(t_{n+1} )-\frac{3}{16}k_1\Delta t -\frac{9}{16}k_4\Delta t , t_{n+1}-\frac34\Delta t ),\\
  &k_6 = a( x(t_{n+1} )+\frac37k_1\Delta t-\frac27k_2\Delta t-\frac{12}{7}k_3\Delta t+\frac{12}{7}k_4\Delta t+\frac87k_5\Delta t   ,t_n  ).
  \end{split}
  \end{equation*}
%  \subsection{Proof of \eqref{eq：e1}}
%  Without loss of generality, we assume the coordinate of vertex  $v_2$ is $(0,0)$ and boundary curve $g(y)$ of $A_j^{\star\star}$ connecting $v_2$ and $v_3$ is positive, see Figure \ref{}.
%  Below, we consider the integral of $(u^{n+1}_j(\bx))^2$ on the region $B$ bounded by the straight line $v_2v_3$ and curve $g(y)$ as follows.
%  \begin{equation}
%  \int_B \left(u^{n+1}_j(\bx)\right)^2 d\bx = \int_0^{h}dy\left(\int_0^{g(y)}\left(u^{n+1}_j(x,y)\right)^2\right)dx.
%  \end{equation}
%  Note that $u^{n+1}_j(x,y)$ is a $P^1$ polynomial, then
%    \begin{align}
%    \notag
%   &\int_0^{h}dy\left(\int_0^{g(y)}\left(u^{n+1}_j(x,y)\right)^2\right)dx\\
%   =&\int_0^{h}dy\left(\int_0^{g(y)}\left(u^{n+1}_j(0,y)\right)^2 + xu^{n+1}_j(0,y)\frac{\partial u^{n+1}_j}{\partial x}(0,y) + \frac{x^2}{2}\left(\frac{\partial u^{n+1}_j}{\partial x}(0,y)\right)^2dx\right).\label{eq:app1}
%    \end{align}
%    We consider the first term on the right hand side. Under the assumption $g(y)\le C_0h^2$
%    \begin{align}
%    \int_0^{h}dy\int_0^{g(y)}\left(u^{n+1}_j(0,y)\right)^2 dx \le C_0h^2\int_0^{h}\left(u^{n+1}_j(0,y)\right)^2 dy \le C_1h\|u_j^{n+1}\|^2_{L^2(A_j)},
%    \end{align}
%    where the trace inequality and the inverse inequality have been applied. The second and third  terms can be treated similarly and we have
%    \begin{equation}
%    \int_B \left(u^{n+1}_j(\bx)\right)^2 d\bx\le C_2 h\|u_j^{n+1}\|^2_{L^2(A_j)}.
%    \end{equation}
%    Therefore, the difference in the $L^2$ norms


%\subsection{Code Architecture}
%
%The code architecture of SLDG is summarized in Figure \ref{class} and Figure\ref{flowchart}.
%In Figure \ref{class}, the class hierarchy of the SLDG code in Rumbaugh notation \cite{blaha2005object} is shown.
%An association indicates an interaction or relation between classes.
%An composition is a stronger form of association in which the composite has sole responsibility for managing its parts.
%An aggregation is an association that represents a part-whole relationship.
%InitialSolution represents ...,
%FinalSolution represents ...,
%NodeOfUpstreamCell represents ...,
%NodeOfEulerianCell represents ...,
%Figure \ref{flowchart} shows a flowchart of SLDG scheme for the transport equation.
%After initialization, the solution on each Eulerian cell, named InitialSolution, can be obtained.
% Firstly, adopting the Runge-Kutta method to solve the ODE with the final value at the node in a Eulerian cell, the node in the corresponding upstream cell, named NodeOfUpstreamCell, can be obtained.
%Then,  a search algorithm is used to obtain the segments on the upstream cell.
% Since the test function is a constant along the characteristic line, its value at a node can be obtained from the corresponding node on the Eulerian cell, and   the test function $\psi^\star(x,y)$ can be reconstructed by interpolation.
% Finally, the area integral is converted to the line integral, and such line integral can be solved analytically.
%
%
%\begin{figure}[h!]
%\centering
%\includegraphics[height=100mm]{Class_Diagram1208}
%\caption{Class hierarchy for the SLDG code using Rumbaugh \cite{blaha2005object} notation. }
%\label{class}
%\end{figure}
%
%
%\begin{figure}[h!]
%\centering
%\includegraphics[height=100mm]{SLDG_flow}
%\caption{Overview of SLDG code for the transport equation.}
%\label{flowchart}
%\end{figure}



==> result.tex <==
\section{Numerical Examples}

In this section, we present the results of our numerical experiments for the schemes described in the previous sections. We will use the third and the fifth order WENO integrations for spatial discretization, denoted as WENO3 and WENO5. And the time discretization $RK(2,3)$ and $RK(4,4)$ are used for WENO3 and WENO5, respectively, to guarantee third order and fourth order accuracy in time. For 1D problems, the time steps are defined as 
$$\Delta t=CFL\Delta x/|c|,$$ 
where $CFL=1.5$ for $RK(2,3)$ and $CFL=2.9$ for $RK(4,4)$. While for 2D problems, the time steps are chosen as
$$\Delta t=CFL/\max(|c_{x}|/\Delta x,|c_{y}|/ \Delta y)$$
where $|c_{x}|$ and $|c_{y}|$ are the maximum wave propagation speeds in the $x$- and $y$-directions, and $\Delta x$ and $\Delta y$ are grid sizes in the $x$- and $y$-directions, respectively. For $RK(2,3)$, we use the third order time splitting scheme \eqref{eq:sp3} with $CFL=1.5$. While, for $RK(4,4)$, we use the forth order time splitting scheme \eqref{eq:sp4} with $CFL=1.6$.

To avoid the effect of rounding error, we change the condition \eqref{eq:pplimiter} into
$$u^n_{i}-\frac{\Delta t}{\Delta x}(\tilde{f}_{i+1/2}-\tilde{f}_{i-1/2})\geq 10^{-16}.$$

\subsection{Basic 1-D and 2-D tests}

\textbf{ Example 4.1} (one-dimensional linear advection equation)
\begin{align}
\label{eq:prob1}
u_{t}+u_{x}=0, \ \ \  x\in [-\pi,\pi]
\end{align}
with two different initial conditions:
\begin{itemize}
\item continuous initial condition $u(x,0)=\cos^4(x)$, 
\item discontinuous initial condition:
$
u(x,0)=\left\{\begin{array}{ll}
1, & x\in[-\frac{1}{4}\pi,\frac{1}{4}\pi]\\
0, & \text{otherwise}.\\
\end{array}
\right.
$
\end{itemize}

The initial condition can be extended periodically on $R$ with period $2\pi$. The exact solution is $u(x,t)=u(x-t,0)$. For the continuous problem, we test with a $2\pi$-periodic boundary condition, a Dirichlet boundary condition $u(-\pi,t)=\cos(-\pi-t)^4$ and a Neumann boundary condition $u_{x}(-\pi,t)=-4\cos(-\pi-t)^3 \sin(-\pi-t)$. The $L_{1}$ and $L_{\infty}$ errors and orders of accuracy are listed in Table \ref{tab1}, \ref{tab2} and \ref{tabadd1}, and the PP-limiter is applied. We observe that WENO3 with $RK(2,3)$ exhibits numerically third order accuracy, as expected. WENO5 with $RK(4,4)$ exhibits the fourth order accuracy. \textcolor{red}{ Note that even though the scheme is fifth order in space, the error in time may dominate the total numerical error due to the large CFL used. If we reduce the CFL less than 1,  fifth order accuracy can be observed. The observed order reduction is similar to that for an Eulerian WENO scheme if a lower order time integrator is coupled.} It is also observed that the PP-limiter is  keep the solutions non-negative without loss of accuracy. While for the discontinuous case (Figure \ref{Fig1}), we consider the $2\pi$-periodic boundary condition and the following Dirichlet boundary condition
\begin{align*}
u(-\pi,t)=\left\{\begin{array}{ll}
1, & t\in[\frac{3}{4}\pi,\frac{5}{4}\pi],\\
0, & t\in(0,\frac{3}{4}\pi)\cup (\frac{5}{4}\pi,2\pi).\\
\end{array}
\right.
\end{align*} 
It is observed that the WENO methodology used effectively suppresses the unphysical oscillations for both schemes.

\textcolor{blue}{Lastly, we would like to investigate numerically the efficiency of the proposed scheme compared with standard Eulerian RKWENO schemes. In particular, we study the numerical errors versus CPU time for the MOL$^T$ WENO5 scheme coupled with implicit $RK(4,4)$ and the Eulerian MOL WENO5 coupled with explicit $RK(4,4)$. Note that both schemes have the same order accuracy in space and time.
The result is summarized in Figure \ref{FigCPU}. We first let $CFL=0.6$, under which both schemes are linearly stable. We observe that the performance of the MOL$^T$ scheme is slightly better than that of the MOL one. We also consider $CFL = 2.9$, which is the upper limit for the MOL$^T$ scheme, while the MOL scheme becomes unstable. We can observe that efficiency of the MOL$^T$ scheme is improved by choosing a larger CFL. Hence, the numerical study demonstrates the advantages of proposed MOL$^T$ approaches for the linear transport problem.}


\begin{table}[htb]
\caption{\label{tab1}\em Accuracy on the one-dimensional linear advection equation with continuous initial condition. $T=2\pi$. Periodic boundary condition. }
\centering
\bigskip
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
  \hline
 &  &  $N_x$ &  $L_1$ errors &   order  &  $L_\infty$ error  & order & min value \\\hline
 \multirow{12}{1.5cm}{WENO3} & \multirow{6}{2cm}{Without\\ PP-limiters}  &
           20 &  6.29E-01  &    --    &  2.36E-01  &     --    &  7.11E-03  \\
 & &    40 &  1.21E-01  &  2.38  &  4.29E-02  &  2.46  &  -7.30E-03  \\
 & &    80 &  1.32E-02  &  3.20  &  4.77E-03  &  3.17  &  -1.48E-03  \\
 & &  160 &  1.25E-03  &  3.39  &  5.21E-04  &  3.19  &  -2.32E-04  \\
 & &  320 &  1.17E-04  &  3.42  &  4.40E-05  &  3.57  &  -2.74E-05  \\
 & &  640 &  1.50E-05  &  2.96  &  4.83E-06  &  3.19  &  -2.89E-06  \\\cline{2-8}
 & \multirow{6}{2cm}{With\\ PP-limiters}  &
 		  20 &  6.28E-01  &    --    &  2.33E-01  &    --     &  1.35E-02  \\
 & &    40 &  1.22E-01  &  2.37  &  4.38E-02  &  2.41  &  1.11E-16  \\
 & &    80 &  1.29E-02  &  3.24  &  4.95E-03  &  3.15  &  1.11E-16  \\
 & &  160 &  1.19E-03  &  3.44  &  4.87E-04  &  3.35  &  1.11E-16  \\
 & &  320 &  1.17E-04  &  3.35  &  5.92E-05  &  3.04  &  1.11E-16  \\
 & &  640 &  1.50E-05  &  2.96  &  8.77E-06  &  2.76  &  1.11E-16  \\\hline
  \multirow{12}{1.5cm}{WENO5} & \multirow{6}{2cm}{Without\\ PP-limiters}  &
           20 &  4.17E-01  &    --    &  1.57E-01  &     --    &  -4.28E-02  \\
 & &    40 &  3.63E-02  &  3.52  &  1.95E-02  &  3.01  &  -5.50E-03  \\
 & &    80 &  2.26E-03  &  4.01  &  1.32E-03  &  3.89  &  -4.79E-05  \\
 & &  160 &  1.24E-04  &  4.19  &  8.48E-05  &  3.96  &  -6.48E-06  \\
 & &  320 &  5.49E-06  &  4.50  &  2.05E-06  &  5.37  &  -3.83E-07  \\
 & &  640 &  3.26E-07  &  4.08  &  8.86E-08  &  4.53  &  -1.01E-09  \\\cline{2-8}
 & \multirow{6}{2cm}{With\\ PP-limiters}  &
 		  20 &  5.06E-01  &    --    &  2.00E-01  &    --     &  1.59E-02 \\
 & &    40 &  5.10E-02  &  3.31  &  2.93E-02  &  2.77  &  7.06E-04  \\
 & &    80 &  6.01E-03  &  3.08  &  4.86E-03  &  2.59  &  3.36E-04  \\
 & &  160 &  1.55E-04  &  5.28  &  1.28E-04  &  5.25  &  7.28E-06  \\
 & &  320 &  5.43E-06  &  4.84  &  1.75E-06  &  6.19  &  4.75E-08  \\
 & &  640 &  3.26E-07  &  4.06  &  8.86E-08  &  4.30  &  1.73E-10  \\\hline
\end{tabular}
\end{small}
\end{table}


\begin{table}[htb]
\caption{\label{tab2}\em Accuracy on the one-dimensional linear advection equation with continuous initial condition. $T=2\pi$. Dirichlet boundary condition. }
\centering
\bigskip
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
  \hline
 &  &  $N_x$ &  $L_1$ errors &   order  &  $L_\infty$ error  & order & min value \\\hline
 \multirow{12}{1.5cm}{WENO3} & \multirow{6}{2cm}{Without\\ PP-limiters}  &
     	  20 &  4.55E-01  &    --     &  3.11E-01  &    --    &  -4.42E-03  \\
 & &    40 &  9.09E-02  &  2.32  &  6.66E-02  &  2.22  &  -1.28E-03  \\
 & &    80 &  1.10E-02  &  3.05  &  1.15E-02  &  2.54  &  -3.71E-04  \\
 & &  160 &  1.08E-03  &  3.35  &  2.46E-03  &  2.22  &  -1.09E-04  \\
 & &  320 &  8.87E-05  &  3.60  &  1.95E-04  &  3.66  &  -1.82E-05  \\
 & &  640 &  9.63E-06  &  3.20  &  6.09E-06  &  5.00  &  -2.15E-06  \\\cline{2-8}
  & \multirow{6}{2cm}{With\\ PP-limiters}  &
      	  20 &  4.53E-01  &    --     &  3.11E-01  &    --    &  1.11E-16  \\
 & &    40 &  9.07E-02  &  2.32  &  6.66E-02  &  2.22  &  5.55E-17  \\
 & &    80 &  1.10E-02  &  3.04  &  1.15E-02  &  2.54  &  5.55E-17  \\
 & &  160 &  1.06E-03  &  3.38  &  2.46E-03  &  2.22  &  5.55E-17  \\
 & &  320 &  8.87E-05  &  3.58  &  1.95E-04  &  3.66  &  1.11E-16  \\
 & &  640 &  9.63E-06  &  3.20  &  6.61E-06  &  4.88  &  5.55E-17  \\
\hline
 \multirow{12}{1.5cm}{WENO5} & \multirow{6}{2cm}{Without\\ PP-limiters}  &
     	  20 &  3.59E-01  &    --    &  2.14E-01  &     --    &  1.18E-02  \\
 & &    40 &  4.37E-02  &  3.04  &  3.24E-02  &  2.73  &  9.44E-04  \\
 & &    80 &  2.65E-03  &  4.05  &  5.79E-03  &  2.48  &  1.98E-05  \\
 & &  160 &  1.08E-04  &  4.61  &  1.69E-04  &  5.10  &  -1.52E-06  \\
 & &  320 &  2.91E-06  &  5.22  &  1.70E-06  &  6.64  &  -1.99E-07  \\
 & &  640 &  1.69E-07  &  4.10  &  8.22E-08  &  4.37  &  6.37E-09  \\\cline{2-8}
  & \multirow{6}{2cm}{With\\ PP-limiters}  &
  	      20 &  3.58E-01  &    --     &  2.15E-01  &    --    &  1.18E-02  \\
 & &    40 &  4.37E-02  &  3.04  &  3.24E-02  &  2.73  &  1.29E-03  \\
 & &    80 &  2.83E-03  &  3.95  &  5.79E-03  &  2.48  &  3.53E-05  \\
 & &  160 &  1.18E-04  &  4.57  &  1.75E-04  &  5.05  &  6.26E-06  \\
 & &  320 &  2.89E-06  &  5.36  &  1.67E-06  &  6.71  &  1.11E-16  \\
 & &  640 &  1.69E-07  &  4.10  &  8.22E-08  &  4.35  &  6.37E-09  \\
\hline
\end{tabular}
\end{small}
\end{table}



\begin{table}[htb]
\caption{\label{tabadd1}\em Accuracy on the one-dimensional linear advection equation with continuous initial condition. $T=2\pi$. Neumann boundary condition. }
\centering
\bigskip
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
  \hline
 &  &  $N_x$ &  $L_1$ errors &   order  &  $L_\infty$ error  & order & min value \\\hline
 \multirow{12}{1.5cm}{WENO3} & \multirow{6}{2cm}{Without\\ PP-limiters}  &
           20 &  4.52E-01  &    --    &  3.09E-01  &     --    &  -7.98E-03  \\
 & &    40 &  9.14E-02  &  2.31  &  6.65E-02  &  2.22  &  -1.22E-03  \\
 & &    80 &  1.11E-02  &  3.05  &  1.15E-02  &  2.54  &  -4.02E-04  \\
 & &  160 &  1.09E-03  &  3.34  &  2.46E-03  &  2.22  &  -1.10E-04  \\
 & &  320 &  9.09E-05  &  3.58  &  1.95E-04  &  3.66  &  -1.83E-05  \\
 & &  640 &  9.93E-06  &  3.20  &  6.09E-06  &  5.00  &  -2.16E-06  \\\cline{2-8}
 & \multirow{6}{2cm}{With\\ PP-limiters}  &
 		  20 &  4.50E-01  &    --    &  3.09E-01  &    --     &  1.11E-16  \\
 & &    40 &  9.12E-02  &  2.30  &  6.64E-02  &  2.22  &  5.55E-17  \\
 & &    80 &  1.12E-02  &  3.04  &  1.15E-02  &  2.54  &  5.55E-17  \\
 & &  160 &  1.07E-03  &  3.37  &  2.46E-03  &  2.22  &  5.55E-17  \\
 & &  320 &  9.10E-05  &  3.56  &  1.95E-04  &  3.66  &  1.11E-16  \\
 & &  640 &  9.93E-06  &  3.20  &  6.65E-06  &  4.87  &  5.55E-17  \\\hline
  \multirow{12}{1.5cm}{WENO5} & \multirow{6}{2cm}{Without\\ PP-limiters}  &
           20 &  3.92E-01  &    --    &  2.22E-01  &     --    &  -2.93E-02  \\
 & &    40 &  4.75E-02  &  3.05  &  3.18E-02  &  2.80  &  -1.87E-03  \\
 & &    80 &  5.02E-03  &  3.24  &  5.74E-03  &  2.47  &  -4.70E-05  \\
 & &  160 &  3.13E-04  &  4.01  &  6.20E-04  &  3.21  &   9.64E-06  \\
 & &  320 &  4.11E-06  &  6.25  &  1.91E-06  &  8.34  &  -4.50E-07  \\
 & &  640 &  2.51E-07  &  4.03  &  1.20E-07  &  4.00  &  -1.00E-08  \\\cline{2-8}
 & \multirow{6}{2cm}{With\\ PP-limiters}  &
 		  20 &  3.95E-01  &    --    &  2.45E-01  &    --     &  4.85E-03 \\
 & &    40 &  5.74E-02  &  2.78  &  4.93E-02  &  2.31  &  0.00E+00  \\
 & &    80 &  6.32E-03  &  3.18  &  6.80E-03  &  2.86  &  1.56E-04  \\
 & &  160 &  2.35E-04  &  4.75  &  4.00E-04  &  4.09  &  1.28E-05  \\
 & &  320 &  3.93E-06  &  5.90  &  1.91E-06  &  7.71  &  1.11E-16  \\
 & &  640 &  2.29E-07  &  4.10  &  1.20E-07  &  4.00  &  0.00E+00  \\\hline
\end{tabular}
\end{small}
\end{table}



\begin{figure}
\centering
\subfigure[Periodic boundary condition.]{
\includegraphics[width=0.4\textwidth]{1d_per}}
\subfigure[Dirichlet boundarycondition.]{
\includegraphics[width=0.4\textwidth]{1d_dir}}
\caption{\em The one-dimensional linear advection equation with discontinuous initial condition. $T=2\pi$. $100$ grid points.}
\label{Fig1}
\end{figure}

\begin{figure}
	\centering
		\includegraphics[width=0.4\textwidth]{CPU}
	\caption{\em Comparison of CPU time against $L_1$ error for the one-dimensional linear advection equation with continuous initial condition and periodic boundary conditions. $T=2\pi$.}
	\label{FigCPU}
\end{figure}


\textbf{Example 4.2} (Rigid body rotation)
\begin{align}
\label{eq:prob2}
u_{t}+yu_{x}-xu_{y}=0, \ \ \ x,y\in\Omega
\end{align}
with two different initial conditions:
\begin{itemize}
\item
continuous initial condition, with $\Omega=[-\frac{1}{2}\pi,\frac{1}{2}\pi]^2$
\begin{align*}
u(x,y,0)=0.5B(\sqrt{x^2+8y^2})+0.5B(\sqrt{8x^2+y^2}),
\end{align*}
where
$
B(r)=\left\{\begin{array}{ll}
\cos(r)^6,& \text{if} \ r\leq \frac{1}{2}\pi,\\
0, & \text{otherwise}.\\
\end{array}
\right.
$

\item dicontinuous initial condition, with $\Omega=[-1,1]^2$
\begin{align*}
u(x,y,0)=\left\{\begin{array}{ll}
1, & (x,y)\in[-0.75,0.75]\times[-0.25,0.25]\bigcup[-0.25,0.25]\times[-0.75,0.75],\\
0, & \text{otherwise}.\\
\end{array}
\right.
\end{align*}
\end{itemize}

We simulate both problems with the zero Dirichlet boundary conditions. In Table \ref{tab4}, we summarize the convergence study and minimum solution values at the final time $T=2\pi$. It is observed  that our schemes can achieve the designed order of accuracy, and meanwhile the PP-limiter is able to preserve positivity without destroying the accuracy of the original scheme. Furthermore, similar to the 1D case, the WENO methodology removes unphysical oscillations as expected (Figure \ref{Fig2}).


%\begin{table}[htb]
%\caption{\label{tab3}\em Errors and orders of accuracy for solving \eqref{eq:prob2} with continuous initial condition at $T=2\pi$. Periodic boundary condition.}
%\centering
%\bigskip
%\begin{small}
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%  \hline
% &  &  $N_x\times N_y$ &  $L_1$ errors &   order  &  $L_\infty$ error  & order & min value \\\hline
% \multirow{10}{1.5cm}{WENO3} & \multirow{5}{2cm}{Without\\ PP-limiters}  &
%      	   $20\times20$ &  2.51E-01  &    --    &  4.25E-01  &    --     &  4.02E-03  \\
% & &     $40\times40$ &  1.14E-01  &  1.14  &  1.72E-01  &  1.31  &  -4.03E-04  \\
% & &     $80\times80$ &  2.89E-02  &  1.98  &  3.35E-02  &  2.36  &  -1.80E-03  \\
% & & $160\times160$ &  3.82E-03  &  2.92  &  4.40E-03  &  2.93  &  -4.68E-04  \\
% & & $320\times320$ &  4.09E-04  &  3.23  &  5.20E-04  &  3.08  &  -7.25E-05  \\\cline{2-8}
% & \multirow{5}{2cm}{With\\ PP-limiters}  &
%      	   $20\times20$ &  2.51E-01  &    --    &  4.25E-01  &    --     &  4.02E-03  \\
% & &     $40\times40$ &  1.14E-01  &  1.14  &  1.72E-01  &  1.31  &  9.98E-17  \\
% & &     $80\times80$ &  2.52E-02  &  2.18  &  3.34E-02  &  2.37  &  1.00E-16  \\
% & & $160\times160$ &  3.37E-03  &  2.90  &  4.40E-03  &  2.92  &  1.00E-16  \\
% & & $320\times320$ &  4.09E-04  &  3.04  &  5.20E-04  &  3.08  &  1.00E-16  \\\hline
% \multirow{10}{1.5cm}{WENO5} & \multirow{5}{2cm}{Without\\ PP-limiters}  &
%            $20\times20$ &  1.82E-01  &    --    &  3.32E-01  &   --      &  8.47E-04   \\  	
% & &     $40\times40$ &  6.26E-02  &  1.54  &  7.43E-02  &  2.16  &  -1.21E-03  \\
% & &     $80\times80$ &  5.10E-03  &  3.62  &  7.49E-03  &  3.31  &  -6.88E-05  \\
% & & $160\times160$ &  1.53E-04  &  5.05  &  2.75E-04  &  4.77  &  -4.76E-06  \\
% & & $320\times320$ &  4.13E-06  &  5.22  &  7.56E-06  &  5.18  &  -1.03E-07  \\\cline{2-8}
% & \multirow{5}{2cm}{With\\ PP-limiters}  &
%           $20\times20$ &  1.82E-01  &   --     &  3.32E-01  &    --     &  8.47E-04  \\  	
% & &     $40\times40$ &  6.19E-02  &  1.56  &  7.43E-02  &  2.16  &  1.00E-16  \\
% & &     $80\times80$ &  5.06E-03  &  3.61  &  7.50E-03  &  3.31  &  1.00E-16  \\
% & & $160\times160$ &  1.52E-04  &  5.06  &  2.75E-04  &  4.77  &  1.00E-16  \\
% & & $320\times320$ &  4.10E-06  &  5.21  &  7.56E-06  &  5.18  &  1.00E-16  \\
%  \hline
%\end{tabular}
%\end{small}
%\end{table}


\begin{table}[htb]
\caption{\label{tab4}\em Accuracy on the rigid body rotation with continuous initial condition. $T=2\pi$.}
\centering
\bigskip
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
  \hline
 &  &  $N_x\times N_y$ &  $L_1$ errors &   order  &  $L_\infty$ error  & order & min value \\\hline
 \multirow{10}{1.5cm}{WENO3} & \multirow{5}{2cm}{Without\\ PP-limiters}  &
 	       $20\times20$ &  1.84E-01  &     --    &  4.25E-01  &   --     &  -2.22E-05  \\
 & &     $40\times40$ &  9.84E-02  &  0.90  &  1.72E-01  &  1.31  &  -1.41E-04  \\
 & &     $80\times80$ &  2.66E-02  &  1.89  &  3.35E-02  &  2.36  &  -2.46E-04  \\
 & & $160\times160$ &  3.41E-03  &  2.96  &  4.40E-03  &  2.93  &  -2.84E-04  \\
 & & $320\times320$ &  3.96E-04  &  3.10  &  5.20E-04  &  3.08  &  -7.25E-05  \\\cline{2-8}
 & \multirow{5}{2cm}{With\\ PP-limiters}  &
 	       $20\times20$ &  1.84E-01  &     --    &  4.25E-01  &    --     &  0.00E+00  \\
 & &     $40\times40$ &  9.84E-02  &  0.90  &  1.72E-01  &  1.31  &  0.00E+00  \\
 & &     $80\times80$ &  2.65E-02  &  1.89  &  3.35E-02  &  2.36  &  0.00E+00  \\
 & & $160\times160$ &  3.32E-03  &  3.00  &  4.40E-03  &  2.93  &  0.00E+00  \\
 & & $320\times320$ &  3.92E-04  &  3.09  &  5.20E-04  &  3.08  &  0.00E+00  \\\hline
 \multirow{10}{1.5cm}{WENO5} & \multirow{5}{2cm}{Without\\ PP-limiters}  &
     	   $20\times20$ &  1.43E-01  &    --    &  3.32E-01  &    --     &  -9.51E-07  \\  	
 & &     $40\times40$ &  6.08E-02  &  1.24  &  7.43E-02  &  2.16  &  -1.67E-05  \\
 & &     $80\times80$ &  4.98E-03  &  3.61  &  7.49E-03  &  3.31  &  -2.50E-05  \\
 & & $160\times160$ &  1.34E-04  &  5.22  &  2.75E-04  &  4.77  &  -4.76E-06  \\
 & & $320\times320$ &  3.73E-06  &  5.16  &  7.56E-06  &  5.18  &  -1.03E-07  \\\cline{2-8}
 & \multirow{5}{2cm}{With\\ PP-limiters}  &
     	   $20\times20$ &  1.43E-01  &    --     &  3.32E-01  &    --    &  0.00E+00  \\  	
 & &     $40\times40$ &  6.09E-02  &  1.24  &  7.43E-02  &  2.16  &  0.00E+00  \\
 & &     $80\times80$ &  4.98E-03  &  3.61  &  7.49E-03  &  3.31  &  0.00E+00  \\
 & & $160\times160$ &  1.34E-04  &  5.22  &  2.75E-04  &  4.77  &  0.00E+00  \\
 & & $320\times320$ &  3.72E-06  &  5.17  &  7.56E-06  &  5.18  &  0.00E+00  \\
  \hline
\end{tabular}
\end{small}
\end{table}


%\begin{table}[htb]
%\caption{\label{tabadd2}\em Errors and orders of accuracy for solving \eqref{eq:prob2} with continuous initial condition at $T=2\pi$. Neumann boundary condition.}
%\centering
%\bigskip
%\begin{small}
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%  \hline
% &  &  $N_x\times N_y$ &  $L_1$ errors &   order  &  $L_\infty$ error  & order & min value \\\hline
% \multirow{10}{1.5cm}{WENO3} & \multirow{5}{2cm}{Without\\ PP-limiters}  &
% 	       $20\times20$ &  1.85E-01  &     --    &  4.25E-01  &   --     &  -2.37E-05  \\
% & &     $40\times40$ &  9.86E-02  &  0.90  &  1.72E-01  &  1.31  &  -4.00E-04  \\
% & &     $80\times80$ &  2.66E-02  &  1.89  &  3.35E-02  &  2.36  &  -2.70E-04  \\
% & & $160\times160$ &  3.47E-03  &  2.94  &  4.40E-03  &  2.93  &  -5.53E-04  \\
% & & $320\times320$ &  6.92E-04  &  2.33  &  8.77E-04  &  2.33  &  -7.25E-05  \\\cline{2-8}
% & \multirow{5}{2cm}{With\\ PP-limiters}  &
% 	       $20\times20$ &  1.84E-01  &     --    &  4.25E-01  &    --     &  0.00E+00  \\
% & &     $40\times40$ &  9.84E-02  &  0.90  &  1.72E-01  &  1.31  &  0.00E+00  \\
% & &     $80\times80$ &  2.65E-02  &  1.89  &  3.35E-02  &  2.36  &  0.00E+00  \\
% & & $160\times160$ &  3.33E-03  &  3.00  &  4.40E-03  &  2.93  &  0.00E+00  \\
% & & $320\times320$ &  3.89E-04  &  3.10  &  5.20E-04  &  3.08  &  0.00E+00  \\\hline
% \multirow{10}{1.5cm}{WENO5} & \multirow{5}{2cm}{Without\\ PP-limiters}  &
 %    	   $20\times20$ &  1.44E-01  &    --    &  3.32E-01  &    --     &  -4.98E-07  \\  	
 %& &     $40\times40$ &  6.08E-02  &  1.24  &  7.43E-02  &  2.16  &  -1.66E-05  \\
% & &     $80\times80$ &  4.98E-03  &  3.61  &  7.49E-03  &  3.31  &  -2.50E-05  \\
% & & $160\times160$ &  1.34E-04  &  5.22  &  2.75E-04  &  4.77  &  -4.76E-06  \\
% & & $320\times320$ &  3.73E-06  &  5.16  &  7.56E-06  &  5.18  &  -1.03E-07  \\\cline{2-8}
% & \multirow{5}{2cm}{With\\ PP-limiters}  &
%     	   $20\times20$ &  1.44E-01  &    --     &  3.32E-01  &    --    &  0.00E+00  \\  	
% & &     $40\times40$ &  6.09E-02  &  1.24  &  7.43E-02  &  2.16  &  0.00E+00  \\
% & &     $80\times80$ &  4.98E-03  &  3.61  &  7.49E-03  &  3.31  &  0.00E+00  \\
% & & $160\times160$ &  1.34E-04  &  5.22  &  2.75E-04  &  4.77  &  0.00E+00  \\
% & & $320\times320$ &  3.72E-06  &  5.17  &  7.56E-06  &  5.18  &  0.00E+00  \\
%  \hline
%\end{tabular}
%\end{small}
%\end{table}



\begin{figure}
\centering
%\subfigure[WENO3.]{
%\includegraphics[width=0.4\textwidth]{2d_per_rk23}}
\subfigure[WENO3.]{
\includegraphics[width=0.4\textwidth]{2d_dir_rk23}}
%\subfigure[WENO5.]{
%\includegraphics[width=0.4\textwidth]{2d_per_rk44}}
\subfigure[WENO5.]{
\includegraphics[width=0.4\textwidth]{2d_dir_rk44}}
\caption{\em The rigid body rotation with discontinuous initial condition. $T=2\pi$. $100\times100$ grid points.}
%Left: periodic boundary condition; right: Dirichlet boundary condition.}
\label{Fig2}
\end{figure}

\subsection{The VP systems} 

In this subsection, we consider the Vlasov-Poisson equation \eqref{eq:vp} with the following four initial conditions:
\begin{itemize}

\item Strong Landau damping:
\begin{align*}
f(x,v,0)=\frac{1}{\sqrt{2\pi}}(1+\alpha\cos(kx))\exp(-\frac{v^2}{2}), 
x\in[0,L], \ v\in[-V_{c},V_{c}]
\end{align*}
where $\alpha=0.5$, $k=0.5$, $L=4\pi$ and $V_{c}=2\pi$.

\item Two-stream instability I:
\begin{align*}
f(x,v,0)=\frac{2}{7\sqrt{2\pi}} (1+5v^2)(1+\alpha((\cos(2kx)+\cos(3kx))/1.2 +cos(kx))) \exp(-\frac{v^2}{2}), \\
x\in[0,L], \ v\in[-V_{c},V_{c}]
\end{align*}
where $\alpha=0.01$, $k=0.5$, $L=4\pi$ and $V_{c}=2\pi$.

\item Two-stream instability II:
\begin{align*}
f(x,v,0)=\frac{1}{\sqrt{2\pi}} (1+\alpha\cos(kx))v^2 \exp(-\frac{v^2}{2}), \ \ \ 
x\in[0,L], \ v\in[-V_{c},V_{c}]
\end{align*}
where $\alpha=0.05$, $k=0.5$,  $L=4\pi$ and $V_{c}=2\pi$.

\item Bump-on-tail instability:
\begin{align*}
f(x,v,0)=\frac{1}{\sqrt{2\pi}}(1+\alpha\cos(kx)) (0.9\exp(-0.5v^2)+0.2\exp(-4(v-4.5)^2)) \nonumber\\
x\in[-L,L], \ v\in[-V_{c},V_{c}]
\end{align*}
where $\alpha=0.04$, $k=0.3$,  $L=\frac{10}{3}\pi$ and $V_{c}=10$.
\end{itemize}

In our numerical tests, periodic boundary conditions are imposed in both directions, and a fast Fourier transform (FFT) is used to solve the 1-D Poisson's equation. The VP system is time-reversible, meaning that if the solution $f$ is first evolved to time $T/2$, at when we reverse the solution in $v$-direction, i.e., $\tilde{f}(x,v,\frac{1}{2}T)=f(x,-v,\frac{1}{2}T)$, and continue to evolve the reversed solution $\tilde{f}$ to time $T$, then we can recover the initial condition with reverse velocity field, i.e., $\tilde{f}(x,v,T)=f(x,-v,0)$. Below, we make use of such a property of the VP system to perform the accuracy test.
In Table \ref{tab5}-\ref{tab8}, we list the errors of $\tilde{f}(x,-v,T)$ and associated orders of accuracy at time $T=10$, without or with the PP-limiter. As expected, all schemes achieve the designed order accuracy and the limiter does not adversely affect the accuracy. 


Below, we briefly recall some conservation results for the VP system. We hope that our numerical solutions can conserve these physical invariants as much as possible.
\begin{align*}
& Mass=\int_{v}\int_{x} f(x,v,t) dxdv,\\
& \|f\|_{L_{p}}=(\int_{v}\int_{x} |f(x,v,t)|^{p} dxdv)^{1/p}, \ \ \ 1\leq p< \infty, \\
& Energy= \frac{1}{2}(\int_{v}\int_{x}f(x,v,t)v^2dxdv+\int_{x}E^{2}(x,t)dx), \\
& Momentum= \int_{v}\int_{x} f(x,v,t)vdxdv.
\end{align*}

For all problems, we observe that the WENO5 scheme numerically performs better than the WENO3 scheme, showed in Figure \ref{Fig3}-\ref{Fig10}. It is observed that both schemes conserve $L_{1}$ norm (Figure \ref{Fig13}) up to the machine error, since the scheme are both conservative and positivity-preserving if the PP-limiter is applied.
While the WENO5 scheme does a better job in conserving the energy, $L_2$ norm and momentum than the WENO3 scheme. 

%Because the solutions are smooth for all four cases, the SSP condition can be ignored here and non-SSP scheme with larger time step is allowd.

 We test Two-stream instability I with second order central difference scheme in time, which is non-conditionally stable and conditionally SSP.  CFL is taken as 10 such that the scheme is stable but not SSP. In space, we use WENO5. In Figure \ref{Fig17}, we can observe that the scheme simulates the structures well. We remark that the SSP property is not always desired for the VP simulations, especially when the solution is smooth.


\begin{table}[htb]
\caption{\label{tab5}\em Accuracy on strong Landau damping. $T=10$.}
\centering
\bigskip
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
  \hline
 &  &  $N_x\times N_v$ &  $L_1$ errors &   order  &  $L_\infty$ error  & order & min value \\\hline
 \multirow{8}{1.5cm}{WENO3} & \multirow{4}{2cm}{Without\\ PP-limiters}  &
	       $32\times64$ &  1.49E+00  &   --     &  8.98E-02  &    --     & -1.00E-04  \\  		
 & &   $64\times128$ &  3.04E-01  &  2.30  &  2.37E-02  &  1.92  &  -8.67E-05  \\
 & & $128\times256$ &  3.78E-02  &  3.01  &  3.56E-03  &  2.73  &  -3.48E-05  \\
 & & $256\times512$ &  4.43E-03  &  3.09  &  4.05E-04  &  3.14  &  -5.84E-06  \\\cline{2-8}
 & \multirow{4}{2cm}{With\\ PP-limiters}  &
	       $32\times64$ &  1.49E+00  &   --     &  8.98E-02  &    --     &  9.99E-17  \\  		
 & &   $64\times128$ &  3.03E-01  &  2.30  &  2.37E-02  &  1.92  &  1.00E-16  \\
 & & $128\times256$ &  3.78E-02  &  3.01  &  3.56E-03  &  2.73  &  1.00E-16  \\
 & & $256\times512$ &  4.44E-03  &  3.09  &  4.05E-04  &  3.14  &  1.00E-16  \\\hline
 \multirow{8}{1.5cm}{WENO5} & \multirow{4}{2cm}{Without\\ PP-limiters}  &
    		   $32\times64$ &  5.70E-01  &   --     &  4.28E-02  &    --     &  -1.79E-04  \\  		
 & &   $64\times128$ &  4.32E-02  &  3.72  &  5.02E-03  &  3.09  &  -1.47E-05  \\
 & & $128\times256$ &  1.46E-03  &  4.89  &  1.87E-04  &  4.75  &  -2.17E-06  \\
 & & $256\times512$ &  3.98E-05  &  5.19  &  4.82E-06  &  5.28  &  -1.38E-07  \\\cline{2-8}
 & \multirow{4}{2cm}{With\\ PP-limiters}  &
    		   $32\times64$ &  5.70E-01  &    --    &  4.28E-02  &    --     &  1.00E-16  \\  		
 & &   $64\times128$ &  4.31E-02  &  3.72  &  5.02E-03  &  3.09  &  1.00E-16  \\
 & & $128\times256$ &  1.46E-03  &  4.88  &  1.87E-04  &  4.74  &  1.00E-16  \\
 & & $256\times512$ &  4.01E-05  &  5.19  &  4.83E-06  &  5.28  &  1.00E-16  \\\hline
\end{tabular}
\end{small}
\end{table}


\begin{table}[htb]
\caption{\label{tab6}\em Accuracy on two-stream instability I. $T=10$.}
\centering
\bigskip
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
  \hline
 &  &  $N_x\times N_v$ &  $L_1$ errors &   order  &  $L_\infty$ error  & order & min value \\\hline
 \multirow{8}{1.5cm}{WENO3} & \multirow{4}{2cm}{Without \\ PP-limiters}  &
  		   $32\times64$ &  7.17E-02  &   --     &  3.56E-03  &    --     &  -3.47E-06  \\  	
 & &   $64\times128$ &  9.39E-03  &  2.93  &  4.03E-04  &  3.14  &  -3.87E-06  \\
 & & $128\times256$ &  1.05E-03  &  3.17  &  4.51E-05  &  3.16  &  -4.88E-07  \\
 & & $256\times512$ &  1.27E-04  &  3.05  &  5.44E-06  &  3.05  &  1.45E-08  \\\cline{2-8}
 & \multirow{4}{2cm}{With \\ PP-limiters}  &
  		   $32\times64$ &  7.18E-02  &   --     &  3.56E-03  &    --     &  1.00E-16  \\  	
 & &   $64\times128$ &  9.38E-03  &  2.94  &  4.03E-04  &  3.14  &  1.00E-16  \\
 & & $128\times256$ &  1.05E-03  &  3.16  &  4.51E-05  &  3.16  &  1.00E-16  \\
 & & $256\times512$ &  1.27E-04  &  3.05  &  5.44E-06  &  3.05  &  1.45E-08  \\
  \hline
 \multirow{8}{1.5cm}{WENO5} & \multirow{4}{2cm}{Without \\ PP-limiters}  &
  		   $32\times64$ &  3.27E-02  &   --     &  1.44E-03  &    --     &  2.58E-07  \\  		
 & &   $64\times128$ &  1.13E-03  &  4.86  &  5.75E-05  &  4.65  &  -1.21E-07  \\
 & & $128\times256$ &  2.51E-05  &  5.49  &  1.84E-06  &  4.97  &  8.42E-08  \\
 & & $256\times512$ &  5.61E-07  &  5.49  &  4.49E-08  &  5.35  &  6.75E-08  \\\cline{2-8}  
 & \multirow{4}{2cm}{With \\ PP-limiters}  &
  		   $32\times64$ &  3.27E-02  &   --     &  1.44E-03  &    --     &  2.58E-07  \\  		
 & &   $64\times128$ &  1.13E-03  &  4.86  &  5.75E-05  &  4.65  &  1.00E-16  \\
 & & $128\times256$ &  2.51E-05  &  5.49  &  1.84E-06  &  4.97  &  8.42E-08  \\
 & & $256\times512$ &  5.61E-07  &  5.49  &  4.49E-08  &  5.35  &  6.75E-08  \\  
\hline
\end{tabular}
\end{small}
\end{table}



\begin{table}[htb]
\caption{\label{tab7}\em Accuracy on two-stream instability II. $T=10$.}
\centering
\bigskip
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
  \hline
 &  &  $N_x\times N_v$ &  $L_1$ errors &   order  &  $L_\infty$ error  & order & min value \\\hline
 \multirow{8}{1.5cm}{WENO3} & \multirow{4}{2cm}{Without \\ PP-limiters}  &
     	   $32\times64$ &  8.90E-02  &   --     &  4.56E-03  &    --     &  -9.96E-06  \\  	
 & &   $64\times128$ &  9.40E-03  &  3.24  &  5.06E-04  &  3.17  &  -6.65E-06  \\
 & & $128\times256$ &  1.05E-03  &  3.16  &  5.94E-05  &  3.09  &  -8.71E-07  \\
 & & $256\times512$ &  1.22E-04  &  3.10  &  7.06E-06  &  3.07  &  -2.15E-08  \\\cline{2-8}
 & \multirow{4}{2cm}{With \\ PP-limiters}  &
     	   $32\times64$ &  8.92E-02  &   --     &  4.56E-03  &    --     &  1.00E-16  \\  	
 & &   $64\times128$ &  9.38E-03  &  3.25  &  5.06E-04  &  3.17  &  1.00E-16  \\
 & & $128\times256$ &  1.05E-03  &  3.16  &  5.94E-05  &  3.09  &  1.00E-16  \\
 & & $256\times512$ &  1.22E-04  &  3.10  &  7.06E-06  &  3.07  &  1.00E-16  \\\hline
 \multirow{8}{1.5cm}{WENO5} & \multirow{4}{2cm}{Without \\ PP-limiters}  &
     	   $32\times64$ &  7.58E-03  &   --     &  6.37E-04  &    --     &  -3.94E-07  \\  	 	
 & &   $64\times128$ &  2.11E-04  &  5.17  &  2.36E-05  &  4.76  &  -9.53E-07  \\
 & & $128\times256$ &  5.29E-06  &  5.32  &  7.44E-07  &  4.99  &  1.70E-14  \\
 & & $256\times512$ &  1.43E-07  &  5.21  &  2.27E-08  &  5.04  &  2.43E-17  \\\cline{2-8}
 & \multirow{4}{2cm}{With \\ PP-limiters}  &
     	   $32\times64$ &  7.66E-03  &   --     &  6.37E-04  &    --     &  1.00E-16  \\  	 	
 & &   $64\times128$ &  2.17E-04  &  5.14  &  2.36E-05  &  4.76  &  1.00E-16  \\
 & & $128\times256$ &  5.31E-06  &  5.36  &  7.44E-07  &  4.99  &  5.24E-15  \\
 & & $256\times512$ &  1.43E-07  &  5.21  &  2.27E-08  &  5.04  &  1.24E-16  \\\hline
\end{tabular}
\end{small}
\end{table}



\begin{table}[htb]
\caption{\label{tab8}\em Accuracy on bump-on-tail instability. $T=10$. }
\centering
\bigskip
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
  \hline
 &  &  $N_x\times N_v$ &  $L_1$ errors &   order  &  $L_\infty$ error  & order & min value \\\hline
 \multirow{8}{1.5cm}{WENO3} & \multirow{4}{2cm}{Without \\ PP-limiters}  &
 	       $32\times64$ &  5.78E-01  &    --     &  1.97E-02  &   --     &  -1.28E-05  \\  	
 & &   $64\times128$ &  1.10E-01  &  2.39  &  6.36E-03  &  1.63  &  -1.68E-05  \\
 & & $128\times256$ &  1.26E-02  &  3.13  &  8.16E-04  &  2.96  &  -5.76E-07  \\
 & & $256\times512$ &  1.44E-03  &  3.13  &  9.02E-05  &  3.18  &  -5.35E-07  \\\cline{2-8}
 & \multirow{4}{2cm}{With \\ PP-limiters}  &
 	       $32\times64$ &  5.78E-01  &    --     &  1.97E-01  &   --     &  1.00E-16  \\  	
 & &   $64\times128$ &  1.10E-01  &  2.39  &  6.36E-03  &  1.63  &  1.00E-16  \\
 & & $128\times256$ &  1.26E-02  &  3.13  &  8.16E-04  &  2.96  &  1.00E-16  \\
 & & $256\times512$ &  1.44E-03  &  3.13  &  9.02E-05  &  3.18  &  1.00E-16  \\\hline
 \multirow{8}{1.5cm}{WENO5} & \multirow{4}{2cm}{Without \\ PP-limiters}  &
    		   $32\times64$ &  2.25E-01  &    --    &  1.02E-02  &     --    &  -1.23E-06  \\  	 	
 & &   $64\times128$ &  1.66E-02  &  3.76  &  1.44E-03  &  2.83  &  -1.19E-06  \\
 & & $128\times256$ &  7.49E-04  &  4.47  &  7.75E-05  &  4.21  &  -1.31E-06  \\
 & & $256\times512$ &  2.08E-05  &  5.17  &  2.79E-06  &  4.80  &  -1.48E-07  \\\cline{2-8}
 & \multirow{4}{2cm}{With \\ PP-limiters}  &
    		   $32\times64$ &  2.25E-01  &   --     &  1.02E-02  &    --     &  1.00E-16  \\  	 	
 & &   $64\times128$ &  1.66E-02  &  3.76  &  1.44E-03  &  2.83  &  1.00E-16  \\
 & & $128\times256$ &  7.46E-04  &  4.47  &  7.75E-05  &  4.21  &  1.00E-16  \\
 & & $256\times512$ &  2.09E-05  &  5.16  &  2.79E-06  &  4.80  &  1.00E-16  \\\hline
\end{tabular}
\end{small}
\end{table}

\begin{figure}
\centering
\subfigure[$T=10$]{
\includegraphics[width=0.4\textwidth]{RK23,IC1,T=10}}
\subfigure[$T=20$]{
\includegraphics[width=0.4\textwidth]{RK23,IC1,T=20}}
\subfigure[$T=30$]{
\includegraphics[width=0.4\textwidth]{RK23,IC1,T=30}}
\subfigure[$T=40$]{
\includegraphics[width=0.4\textwidth]{RK23,IC1,T=40}}
\caption{\em Strong Landau Damping. WENO3, with $256\times1024$ grid points.}
\label{Fig3}
\end{figure}

\begin{figure}
\centering
\subfigure[$T=10$]{
\includegraphics[width=0.4\textwidth]{RK44,IC1,T=10}}
\subfigure[$T=20$]{
\includegraphics[width=0.4\textwidth]{RK44,IC1,T=20}}
\subfigure[$T=30$]{
\includegraphics[width=0.4\textwidth]{RK44,IC1,T=30}}
\subfigure[$T=40$]{
\includegraphics[width=0.4\textwidth]{RK44,IC1,T=40}}
\caption{\em Strong Landau Damping. WENO5, with $256\times1024$ grid points.}
\label{Fig4}
\end{figure}


\begin{figure}
\centering
\subfigure[$T=10$]{
\includegraphics[width=0.4\textwidth]{RK23,IC2,T=10}}
\subfigure[$T=20$]{
\includegraphics[width=0.4\textwidth]{RK23,IC2,T=20}}
\subfigure[$T=30$]{
\includegraphics[width=0.4\textwidth]{RK23,IC2,T=30}}
\subfigure[$T=40$]{
\includegraphics[width=0.4\textwidth]{RK23,IC2,T=40}}
\caption{\em Two-stream instability I. WENO3, with $256\times1024$ grid points.}
\label{Fig5}
\end{figure}


\begin{figure}
\centering
\subfigure[$T=10$]{
\includegraphics[width=0.4\textwidth]{RK44,IC2,T=10}}
\subfigure[$T=20$]{
\includegraphics[width=0.4\textwidth]{RK44,IC2,T=20}}
\subfigure[$T=30$]{
\includegraphics[width=0.4\textwidth]{RK44,IC2,T=30}}
\subfigure[$T=40$]{
\includegraphics[width=0.4\textwidth]{RK44,IC2,T=40}}
\caption{\em Two-stream instability I. WENO5, with $256\times1024$ grid points.}
\label{Fig6}
\end{figure}

\begin{figure}
\centering
\subfigure[$T=10$]{
\includegraphics[width=0.4\textwidth]{RK12,IC2,T=10}}
\subfigure[$T=20$]{
\includegraphics[width=0.4\textwidth]{RK12,IC2,T=20}}
\subfigure[$T=30$]{
\includegraphics[width=0.4\textwidth]{RK12,IC2,T=30}}
\subfigure[$T=40$]{
\includegraphics[width=0.4\textwidth]{RK12,IC2,T=40}}
\caption{\em Two-stream instability I. Second order centel difference scheme with WENO5. $256\times1024$ grid points.}
\label{Fig17}
\end{figure}

\begin{figure}
\centering
\subfigure[$T=10$]{
\includegraphics[width=0.4\textwidth]{RK23,IC3,T=10}}
\subfigure[$T=20$]{
\includegraphics[width=0.4\textwidth]{RK23,IC3,T=20}}
\subfigure[$T=30$]{
\includegraphics[width=0.4\textwidth]{RK23,IC3,T=30}}
\subfigure[$T=40$]{
\includegraphics[width=0.4\textwidth]{RK23,IC3,T=40}}
\caption{\em Two-stream instability II. WENO3, with $256\times1024$ grid points.}
\label{Fig7}
\end{figure}



\begin{figure}
\centering
\subfigure[$T=10$]{
\includegraphics[width=0.4\textwidth]{RK44,IC3,T=10}}
\subfigure[$T=20$]{
\includegraphics[width=0.4\textwidth]{RK44,IC3,T=20}}
\subfigure[$T=30$]{
\includegraphics[width=0.4\textwidth]{RK44,IC3,T=30}}
\subfigure[$T=40$]{
\includegraphics[width=0.4\textwidth]{RK44,IC3,T=40}}
\caption{\em Two-stream instability II. WENO5, with $256\times1024$ grid points.}
\label{Fig8}
\end{figure}


\begin{figure}
\centering
\subfigure[$T=10$]{
\includegraphics[width=0.4\textwidth]{RK23,IC4,T=10}}
\subfigure[$T=20$]{
\includegraphics[width=0.4\textwidth]{RK23,IC4,T=20}}
\subfigure[$T=30$]{
\includegraphics[width=0.4\textwidth]{RK23,IC4,T=30}}
\subfigure[$T=40$]{
\includegraphics[width=0.4\textwidth]{RK23,IC4,T=40}}
\subfigure[$T=50$]{
\includegraphics[width=0.4\textwidth]{RK23,IC4,T=50}}
\subfigure[$T=60$]{
\includegraphics[width=0.4\textwidth]{RK23,IC4,T=60}}
\caption{\em Bump-on-tail instability. WENO3, with $256\times1024$ grid points.}
\label{Fig9}
\end{figure}



\begin{figure}
\centering
\subfigure[$T=10$]{
\includegraphics[width=0.4\textwidth]{RK44,IC4,T=10}}
\subfigure[$T=20$]{
\includegraphics[width=0.4\textwidth]{RK44,IC4,T=20}}
\subfigure[$T=30$]{
\includegraphics[width=0.4\textwidth]{RK44,IC4,T=30}}
\subfigure[$T=40$]{
\includegraphics[width=0.4\textwidth]{RK44,IC4,T=40}}
\subfigure[$T=50$]{
\includegraphics[width=0.4\textwidth]{RK44,IC4,T=50}}
\subfigure[$T=60$]{
\includegraphics[width=0.4\textwidth]{RK44,IC4,T=60}}
\caption{\em Bump-on-tail instability. WENO5, with $256\times1024$ grid points.}
\label{Fig10}
\end{figure}

\clearpage


%\begin{figure}[H]
%\centering
%\subfigure[Strong Landau damping]{
%\includegraphics[width=0.4\textwidth]{IC1,Mass}}
%\subfigure[Two-stream instability I]{
%\includegraphics[width=0.4\textwidth]{IC2,Mass}}
%\subfigure[Two-stream instability II]{
%\includegraphics[width=0.4\textwidth]{IC3,Mass}}
%\subfigure[Bump-on-tail instability]{
%\includegraphics[width=0.4\textwidth]{IC4,Mass}}
%\caption{\em The time evolution of the relative deviation in total mass. $256\times1024$ grid points. }
%\label{Fig11}
%\end{figure}



\begin{figure}
\centering
\subfigure[Strong-Landau damping]{
\includegraphics[width=0.4\textwidth]{IC1,Energy}}
\subfigure[Two-stream instability I]{
\includegraphics[width=0.4\textwidth]{IC2,Energy}}
\subfigure[Two-stream instability II]{
\includegraphics[width=0.4\textwidth]{IC3,Energy}}
\subfigure[Bump-on-tail instability]{
\includegraphics[width=0.4\textwidth]{IC4,Energy}}
\caption{\em The time evolution of the relative deviation in total energy. $256\times1024$ grid points. }
\label{Fig12}
\end{figure}

\begin{figure}
\centering
\subfigure[Strong Landau damping]{
\includegraphics[width=0.4\textwidth]{IC1,L_1}}
\subfigure[Two-stream instability I]{
\includegraphics[width=0.4\textwidth]{IC2,L_1}}
\subfigure[Two-stream instability II]{
\includegraphics[width=0.4\textwidth]{IC3,L_1}}
\subfigure[Bump-on-tail instability]{
\includegraphics[width=0.4\textwidth]{IC4,L_1}}
\caption{\em The time evolution of the relative deviation in $L_{1}$ norm. $256\times1024$ grid points. }
\label{Fig13}
\end{figure}

\begin{figure}
\centering
\subfigure[Strong Landau damping]{
\includegraphics[width=0.4\textwidth]{IC1,L_2}}
\subfigure[Two-stream instability I]{
\includegraphics[width=0.4\textwidth]{IC2,L_2}}
\subfigure[Two-stream instability II]{
\includegraphics[width=0.4\textwidth]{IC3,L_2}}
\subfigure[Bump-on-tail instability]{
\includegraphics[width=0.4\textwidth]{IC4,L_2}}
\caption{\em The time evolution of the relative deviation in $L_{2}$ norm. $256\times1024$ grid points. }
\label{Fig14}
\end{figure}


\begin{figure}
\centering
\subfigure[Strong Landau damping]{
\includegraphics[width=0.4\textwidth]{IC1,Momentum}}
\subfigure[Two-stream instability I]{
\includegraphics[width=0.4\textwidth]{IC2,Momentum}}
\subfigure[Two-stream instability II]{
\includegraphics[width=0.4\textwidth]{IC3,Momentum}}
\subfigure[Bump-on-tail instability]{
\includegraphics[width=0.4\textwidth]{IC4,Momentum}}
\caption{\em The time evolution of momentum. $256\times1024$ grid points. }
\label{Fig15}
\end{figure}


\subsection{Plasma theath}

Next, we consider the so-called plasma theath problem, which discribes VP system 
with non-periodic boundary condition in x-direction. The initial condition is
\begin{align}
f(x,v,0)=\frac{1}{\sqrt{\alpha\pi}}\exp(-\frac{1}{\alpha}v^2) , \ \ \ x\in[0,L], \ \ \ v\in[-V_{c},V_{c}]
\end{align}
where $\alpha=0.0005526350206$, $L=1$ and $V_{c}=0.2$.
We assume that no electrons can enter the domain, meaning that we take zero-inflow boundary condition: 
\begin{align}
f(x= 0,t, v\geq 0) = f( x= L,t, v\leq 0) = 0.
\end{align}
The electric potential is fixed to a constant value at $x=0$ and $x=L$. Without loss of generality, 
we take $\phi(x=0,t)=\phi(x=L,t)=0$. The solutions at the final time $T=140$ are shown in Figure \ref{Fig16}, with $256\times1024$ grid points. Our results are consistent with that in \cite{seal2012discontinous} .


\begin{figure}
\centering
\subfigure[WENO3]{
\includegraphics[width=0.8\textwidth]{RK23,sh}}
\subfigure[WENO5]{
\includegraphics[width=0.8\textwidth]{RK44,sh}}
\caption{\em Plasma sheath. $256\times1024$ grid points. $T=140$}
\label{Fig16}
\end{figure}

==> test.tex <==
\section{Formulation of the Scheme}

We start with the following one-dimensional advection equation
\begin{equation}\label{eq:1dadv}
  u_t + cu_x = 0,\quad x\in[a,b],
\end{equation}
where $c$ is constant denoting the wave propagation speed. The boundary condition is assumed to be periodic,  Dirichlet boundary condition
$$u(a,t)=g_{1}(t),\ \text{for} \ c>0, \ \ \ \text{or} \ \ \ \ u(b,t)=g_{2}(t),\ \text{for} \ c<0, $$
or  Neumann boundary condition
$$u_{x}(a,t)=h_{1}(t),\ \text{for} \ c>0, \ \ \ \text{or} \ \ \ \ u_{x}(b,t)=h_{2}(t),\ \text{for} \ c<0. $$


\subsection{The method of lines transpose approach}

As discussed in the introduction, in an MOL$^T$ framework, we first discretize the time variable while leaving the spatial variable continuous. For example, we can apply the first order backward Euler method to
\eqref{eq:1dadv}, and obtain
$$
\frac{u^{n+1}-u^n}{\Delta t} + cu^{n+1}_x =0,
$$
i.e.,
\begin{equation}\label{eq:mol1}
  u^{n+1}_x +\text{sgn}(c)\cdot\alpha u^{n+1} =\text{sgn}(c)\cdot\alpha u^n,
\end{equation}
where $\Delta t$ denotes the time step and $\alpha=\frac{1}{|c\Delta t|}$. Note that \eqref{eq:mol1} is an initial value problem (IVP), for which we can obtain an explicit representation for solution $u^{n+1}$ at time level $t^{n+1}$. If we assume $c>0$, $u^{n+1}$ can be represented by
\begin{equation}\label{eq:representationL}
  u^{n+1}(x) = I^L[u^n,\alpha](x) + A^{n+1}e^{-\alpha(x-a)},
\end{equation}
where
\begin{equation}\label{eq:convolutionL}
  I^L[v,\alpha](x) \doteq \alpha\int_a^x e^{-\alpha(x-y)}v(y)dy,
\end{equation}
and $A^{n+1}$ is a constant and should be determined by the boundary condition. The superscript $L$ indicates that the characteristics traverse from the left to the right.
%
If $c<0$, then the characteristics traverse from the right to the left. Due to the symmetry, we can advance the solution as
\begin{equation}\label{eq:representationR}
  u^{n+1}(x) = I^R[u^n,\alpha](x) + B^{n+1}e^{-\alpha(b-x)},
\end{equation}
when the first order backward Euler scheme is used. Here,
\begin{equation}\label{eq:convolutionR}
  I^R[v,\alpha](x) \doteq \alpha\int_x^b e^{-\alpha(y-x)}v(y)dy,
\end{equation}
 and again the constant $B^{n+1}$ is determined by the boundary condition.


We need to further discretize the spatial variable based on the semi-discrete schemes \eqref{eq:representationL} and \eqref{eq:representationR}. Following the idea in \cite{causley,causley2013method}, the domain $[a,b]$ is discretized by $M+1$ uniformly distributed grid points
$$a=x_0<x_1<\cdots<x_{M-1}<x_M=b,$$
and $\Delta x=\frac{b-a}{M}$ denotes the mesh size. The solution is accordingly discretized at points $\{x_i\}_{i=0}^M$, and we use  $u^n_i$ to denote the numerical solution at location $x_i$ at time level $t^n$. The main part of the algorithm is to evaluate the convolution integral $I^{L}[v,\alpha](x)$ in \eqref{eq:representationL}, \eqref{eq:representationR} or $I^{R}[v,\alpha]$ in \eqref{eq:convolutionL}, \eqref{eq:convolutionR} based on the point values $\{v_i\}_{i=0}^M$.

We first consider the case of $c>0$. Note that,
\begin{equation}\label{eq:recursive}
I^L[v,\alpha](x) = I^L[v,\alpha](x-\delta_x)e^{-\alpha\delta_x} + J^L[v,\alpha,\delta_x](x),
\end{equation}
where
\begin{equation}\label{eq:JL}
J^L[v,\alpha,\delta_x](x) \doteq  \alpha\int_{x-\delta_x}^{x} v(y)e^{-\alpha (x-y)}dy,
\end{equation}
and $\delta_x$ is a positive constant.
Therefore, in order to obtain $I^L[v,\alpha](x_i)$ denoted by $I^L_i$,
we only need to approximate the increment $J^L[v,\alpha,\Delta x](x_i)$ denoted by $J^L_i$, then $I^L_i$ is obtained via a recursive relation, i.e.,  %\eqref{eq:recursive}, i.e.,
\begin{equation}\label{eq:recursive1}
I^L_i = I^L_{i-1}e^{-\alpha\Delta x} + J^L_i,\quad i=1,\cdots,M, \quad I^L_0 = 0.
\end{equation}
For the case of $c<0$, again thanks to the symmetry, we have the following identity
\begin{equation}\label{eq:recursive}
I^R[v,\alpha](x) = I^R[v,\alpha](x+\delta_x)e^{-\alpha\delta_x} + J^R[v,\alpha,\delta_x](x),
\end{equation}
where
\begin{equation}\label{eq:JR}
J^R[v,\alpha,\delta_x](x) \doteq  \alpha\int_{x}^{x+\delta_x} v(y)e^{-\alpha (y-x)}dy,
\end{equation}
and hence a similar  recursive relation can be obtained
\begin{equation}\label{eq:recursive2}
I^R_i = I^R_{i+1}e^{-\alpha\Delta x} + J^R_i,\quad i=0,\cdots,M-1, \quad I^R_M = 0,
\end{equation}
where $I^R_i$ and $J^R_i$ denote the approximate values of $I^R[v,\alpha](x_i)$ and $J^R[v,\alpha,\Delta x](x_i)$, respectively.

After computing the contributions from the left or right characteristic, we further need to find the global coefficient $A$ in \eqref{eq:representationL} or $B$ in \eqref{eq:representationR} to enforce the boundary condition.
Since $I^{L}[u^{n},\alpha](a)=I^{R}[u^{n},\alpha](b)=0$, for a Dirichlet boundary condition, the global coefficient can be obtained by
\begin{equation}
\label{eq:bcdir}
A^{n+1}=g_{1}(t^{n+1}), \ \text{or} \ \  B^{n+1}=g_{2}(t^{n+1}).
\end{equation}
Similarly, for a Neumann boundary condition, because $(I^{L}[v,\alpha])'(x)=-\alpha I^{L}[v,\alpha](x)+\alpha v(x)$ and $(I^{R}[v,\alpha])'(x)=\alpha I^{R}[v,\alpha](x)-\alpha v(x)$, we can get the coefficients by
\begin{align}
\label{eq:bcneu}
A^{n+1}=v(a)-\frac{1}{\alpha}h_{1}(t^{n+1}), \ \  \text{or} \ \ 
B^{n+1}=v(b)+\frac{1}{\alpha}h_{2}(t^{n+1}).
\end{align}
For the periodic boundary condition, the coefficient can be determined by using the  mass conservation property of the solution, i.e,
\begin{equation*}
\int_{a}^{b}u(x,t)dx=\int_{a}^{b}u(x,0)dx.
\end{equation*} 
At the discrete level, we enforce
\begin{equation*}
\sum_{i=0}^{M-1}u^{n}_{i}=\sum_{i=0}^{M-1}u^{n+1}_{i}
=\sum_{i=0}^{M-1}I^{L}_{i}+A^{n+1}\sum_{i=0}^{M-1}e^{-i\alpha\Delta x}, \ \ \
u^{n+1}_{M}=u^{n+1}_{0}, \ \ \ for \ c>0,
\end{equation*}
 or 
\begin{equation*}
\sum_{i=1}^{M}u^{n}_{i}=\sum_{i=1}^{M}u^{n+1}_{i}
=\sum_{i=1}^{M}I^{R}_{i}+B^{n+1}\sum_{i=1}^{M}e^{-(M-i)\alpha\Delta x} , \ \ \
u^{n+1}_{0}=u^{n+1}_{M}, \ \ \ for \ c<0.
\end{equation*}
Then the coefficient is obtained
%
\begin{equation}
\label{eq:bcL}
A^{n+1} =\left(\sum_{i=0}^{M-1}u^{n}_{i}-\sum_{i=0}^{M-1}I^{L}_{i}\right)\bigg/\sum_{i=0}^{M-1}e^{-i\alpha\Delta x},
\end{equation}
or
\begin{equation}
\label{eq:bcR}
B^{n+1}=\left(\sum_{i=1}^{M}u^{n}_{i}- \sum_{i=1}^{M}I^{R}_{i}\right)\bigg/ \sum_{i=1}^{M}e^{-(M-i)\alpha\Delta x}.
\end{equation}
\textcolor{red}{Note that we can also impose periodic boundary conditions by letting 
	$$u^{n+1}(a)=u^{n+1}(b),$$
while the total mass may not be automatically conserved.}


\subsection{WENO methodology}

The existing MOL$^T$ schemes mainly rely on linear interpolation methods to compute increment $J^L_i$ and $J^R_i$, see \cite{causley}, which work well for smooth problems. However, the linear schemes may generate spurious oscillations when the solution has discontinuities because of the famous Gibbs phenomenon. In order to control such undesired oscillations, we will incorporate a WENO methodology in the MOL$^T$ framework to evaluate  $J^L_i$ and $J^R_i$ below.

The first WENO scheme was introduced by Liu {\em et al.} \cite{liu1994weighted}, as a third order accurate finite volume scheme to solve hyperbolic conservation laws in one dimension. Later, in \cite{jiang1996efficient}, a general framework for arbitrary order accurate finite difference WENO schemes was designed, which is more efficient for multi-dimensional calculations. The schemes have the advantage of attaining high order accuracy in smooth regions of the solution while maintaining sharp and essentially non-oscillatory transitions of discontinuities. More details about WENO can be found in \cite{shu2009high}.

In our work, a WENO integration procedure is used, based on the idea proposed in \cite{chou2006high,chou2007high,liu2009positivity}. 
Below, a $(2k-1)$-th order approximation of $J^{L}_{i}$ is provided as an example, where $k$ is an integer. The corresponding coefficients of the third order and  fifth order schemes are given in the Appendix. The whole procedure consists of four steps.

\begin{enumerate}
\item
On each small stencil $S_{r}(i)=\{x_{i-r-1},\ldots,x_{i-r-1+k}\}$, $r=0,\ldots,k-1$, which contains $x_{i-1}$ and $x_{i}$, there is a unique polynomial $p_{r}(x)$ of degree at most $k$ which interpolates $v(x)$ at the nodes in $S_{r}(i)$. Then we can get the integral 
\begin{equation}
\label{eq:weno1}
J^{L}_{i,r} =\alpha \int_{x_{i-1}}^{x_{i}}e^{-\alpha(x_{i}-y)}p_{r}(y)dx
=\sum_{j=0}^{k}c^{(r)}_{i-r-1+j}v_{i-r-1+j},
\end{equation}
where the coefficients $c^{(r)}_{i-r-1+j}$ depend on $\alpha$ and the cell size $\Delta x$, but not on $v$.

\item
Similarly, on the big stencil $S(i)=\{x_{i-k},\ldots,x_{i+k-1}\}$, there is a unique polynomial $p(x)$ of degree at most $2k-1$ interpolating $v(x)$ at the nodes in $S(i)$. Then we have
\begin{equation}
\label{eq:weno2}
J^{L}_{i} =\alpha \int_{x_{i-1}}^{x_{i}}e^{-\alpha(x_{i}-y)}p(y)dx
=\sum_{j=0}^{2k-1}c_{i-k+j}v_{i-k+j},
\end{equation}
and linear weights $d_{r}$, such that
\begin{equation}
J^{L}_{i}=\sum_{r=0}^{k-1}d_{r}J^{L}_{i,r},
\end{equation}
where $\sum_{r=0}^{k-1}d_{r}=1$.
\textcolor{blue}{Note that there is no gaurantee that the linear weights are always positive. However,  in our numerical tests, the linear weights are found to be positive all the time. If negative linear weights are present, we can use the idea in \cite{shi2002technique} to address the issue.}

\item
Change the linear weights $d_{r}$ into nonlinear weights $\omega_{r}$, using
\begin{equation}
\omega_{r}=\frac{\tilde{\omega}_{r}}{\sum_{s=0}^{k-1}\tilde{\omega}_{s}}, \ \ r=0,\ldots,k-1,
\end{equation}
with
\begin{equation*}
\tilde{\omega}_{r}=\frac{d_{r}}{(\epsilon+\beta_{r})^2}.
\end{equation*}
Here, $\epsilon>0$ is a small number to avoid the denominator becoming zero, and we take $\epsilon=10^{-6}$ in our numerical tests. The smoothness indicator $\beta_{r}$, measuring the relative smoothness of the function $v(x)$ in the stencil $S_{r}(i)$, is defined by
\begin{equation}
\beta_{r}=\sum_{l=1}^{k} \int_{x_{i-1}}^{x_{i}}\Delta x^{2l-1} (\frac{\partial^{l}p_{r}(x)}{\partial x^{l}})^2 dx.
\end{equation}

 
\item
Lastly, we have 
\begin{equation}
J^{L}_{i}=\sum_{r=0}^{k-1}\omega_{r}J^{L}_{i,r}.
\end{equation}

\end{enumerate}

The process to obtain $J^{R}_{i}$ is mirror-symmetric to that for $J^{L}_{i}$ with respect to the point $x_{i}$.

When dealing with a Dirichlet or a Neumann boundary condition, we further need to extrapolate point values at the ghost points $\{x_{-(k-1)},\ldots,x_{-1}\}$ and $\{x_{M+1},\ldots,x_{M+k-1}\}$ using the point values in the domain, where
$$x_{-i}=x_{0}-i\Delta x, \ \ x_{M+i}=x_{M}+i\Delta x.$$  
Following the idea in \cite{tan2012efficient}, a WENO extrapolation strategy is designed to get more robust results. For instance, when approximating the left ghost point $x_{-i}$, we consider the big stencil $S_{2k-2}=\{x_{0},\ldots,x_{2k-2}\}$:

\begin{enumerate}
\item On each small stencil $S_{r}=\{x_{0},\ldots,x_{r}\}$, $r=0,\ldots,2k-2$, we can construct a polynomial $p_{r}(x)$ of degree at most $r$ interpolating $v(x)$ at the nodes in $S_{r}$. And $v_{-i}$ can be extrapolated by
\begin{align}
v_{-i}=\sum_{r=0}^{2k-2}d_{r}p_{r}(x_{-i}),
\end{align}
where $d_{0}=\Delta x^{2k-2}$, $d_{1}=\Delta x^{2k-3}$, $\ldots$, $d_{2k-3}=\Delta x$, and $d_{2k-2}=1-\sum_{r=0}^{2k-3}d_{r}$.

\item Change the weights $d_{r}$ into nonlinear weights $\omega_{r}$
\begin{equation}
\omega_{r}=\frac{\tilde{\omega}_{r}}{\sum_{s=0}^{2k-2}\tilde{\omega}_{s}}, \ \ r=0,\ldots,2k-2,
\end{equation}
with
\begin{equation*}
\tilde{\omega}_{r}=\frac{d_{r}}{(\epsilon+\beta_{r})^2}.
\end{equation*}
Again, we take $\epsilon=10^{-6}$ in our numerical tests to avoid the denominator becoming zero. And the smoothness indicator $\beta_{r}$ is defined by
\begin{align*}
& \beta_{0}=\Delta x^2,\\
& \beta_{r}=\sum_{l=1}^{r} \int_{x_{-1}}^{x_{0}}\Delta x^{2l-1} (\frac{\partial^{l}p_{r}(x)}{\partial x^{l}})^2 dx, \ \ r=1,\ldots,2k-2.
\end{align*}

\item Finally, we have
\begin{align*}
v_{-i}=\sum_{r=0}^{2k-2}\omega_{r}p_{r}(x_{-i}).
\end{align*}

\end{enumerate} 

Similarly, we can apply the WENO extrapolation to right ghost points $x_{M+i}$ based on stencil $S_{2k-2}=\{x_{M-2k+2},\ldots,x_{M}\}$.



\subsection{High order time discretization}
Note that scheme \eqref{eq:mol1} is first order accurate in time. Below, we will extend our schemes to high order accuracy via the implicit SSP RK method \cite{gottlieb2001strong,ketcheson2009optimal}. 

To approximate the solutions of ordinary differential equation
\begin{equation}
u_{t}=F(u),
\end{equation}
an $s$-stage and $k$-th order RK method, denoted as $RK(s,k)$, is defined as
\begin{subequations}
\label{eq:rk}
\begin{align}
& u^{(i)}=u^{n}+\Delta t\sum_{j=1}^{s}a_{ij}F(u^{(j)},t_{n}+c_{j}\Delta t),   \ \ \ i\leq j\leq s,\\
& u^{n+1}=u^{n}+\Delta t\sum_{j=1}^{s}b_{j}F(u^{(j)},t_{n}+c_{j}\Delta t), 
\end{align}
\end{subequations}
with the standard assumption
\begin{equation*}
c_{i}=\sum_{j=1}^{s}a_{ij}.
\end{equation*}
Denote the matrix $\textbf{A}=(a_{ij})_{s\times s}$ and the vector $\textbf{b}=(b_{i})_{s\times 1}$.
In our scheme, we will use the diagonally implicit (DIRK) methods, for which $\textbf{A}$ is lower triangular.  Denote $\textbf{1}=[1,\ldots,1]^{T}\in R^{s}$, $\textbf{U}^{rk}=[u^{(1)},\ldots, u^{(s)}] ^{T}$, $\textbf{F}=[\Delta t F(u^{(1)},t_{n}+c_{1}\Delta t),\ldots,\Delta tF(u^{(s)},t_{n}+c_{s}\Delta t)]^T$, and $\Lambda=diag(a_{11},\ldots,a_{ss})$. Then, we can get
$\textbf{F}=\textbf{A}^{-1}(\textbf{U}^{rk}-u^{n}\cdot\textbf{1})$. Hence,
\begin{subequations}
\begin{align}
& \textbf{U}^{rk}-\Lambda\cdot\textbf{F}
=u^{n}\cdot\Lambda\cdot\textbf{A}^{-1}\cdot\textbf{1}+ (\textbf{A}-\Lambda)\cdot\textbf{A}^{-1} \textbf{U}^{rk},
\label{eq:rk1}\\
& u^{n+1}=u^{n}+\textbf{b}^{T}\cdot\textbf{F}
=u^{n}+\textbf{b}^{T}\cdot\textbf{A}^{-1}(\textbf{U}^{rk}-u^{n}\cdot\textbf{1}).
\label{eq:rk2}
\end{align}
\end{subequations}
Note that $\textbf{A}$ is lower triangular. So $(\textbf{A}-\Lambda)\cdot\textbf{A}^{-1}$ is also lower triangular, with all diagnal elements equal to zero.  

For problem \eqref{eq:1dadv}, $F(u)=-cu_{x}$. Corresponding, each stage of \eqref{eq:rk1} can be rewritten as
\begin{align}
\label{eq:rkmolt}
u^{(i)}_{x} +\text{sgn}(c\cdot a_{ii}) \alpha_{i} u^{(i)} =\tilde{\alpha}_{i}u^{n}+ \sum_{j=1}^{i-1}\tilde{\alpha}_{ij}u^{(j)},
\end{align}
where $\alpha_{i} = 1/|c\cdot a_{ii}\Delta t|$. We can solve \eqref{eq:rkmolt} with the MOL$^T$ method mentioned above. And finally, $u^{n+1}$ is obtained by \eqref{eq:rk2}.


When considering the periodic boundary condition for problem \eqref{eq:1dadv}, the global coefficients $A^{rk,i}$ or $B^{rk,i}$ on each stage can be obtained by \eqref{eq:bcL} or \eqref{eq:bcR}. For a Dirichlet boundary condition, the scheme may lose accuracy if we define $A^{rk,i}=g_{1}(t_{rk}^{i})$ or $B^{rk,i}=g_{2}(t_{rk}^{i})$. To avoid order reduction, we follow the idea in \cite{Isaia_rkbc}. In particular, denote $\textbf{c}^{l}=[c_{1}^{l},\ldots,c_{s}^{l}]^{T}$ for $l>0$. To achieve $k$-th order of accuracy, boundary values at intermediate stages are defined as
\begin{align}
\textbf{A}^{rk}
=& \sum_{l=0}^{k-2}(\text{A}^{l} \textbf{1} \otimes \Delta t^{l} \textbf{c}^{l})\frac{d^{l}}{dt^{l}} g_{1}(t_{n})
+(\textbf{A}^{k-1}\otimes \Delta t^{k-1}\textbf{c}^{k-1})\frac{d^{k-1}}{dt^{k-1}} \textbf{G}_{1}^{n+c}
\end{align}
for $c>0$, where
\begin{align*}
& \textbf{A}^{rk}=[A^{rk,1},\ldots,A^{rk,s}]^T, \\
& \textbf{G}_{1}^{n+c}=[g_{1}(t^{n}+c_{1}\Delta t),\ldots,g_{1}(t^{n}+c_{s}\Delta t)]^T,
\end{align*}
or
\begin{align}
\textbf{B}^{rk}
=& \sum_{l=0}^{k-2}(\text{A}^{l} \textbf{1} \otimes \Delta t^{l} \textbf{c}^{l})\frac{d^{l}}{dt^{l}} g_{2}(t_{n})
+(\textbf{A}^{k-1}\otimes \Delta t^{k-1}\textbf{c}^{k-1})\frac{d^{k-1}}{dt^{k-1}} \textbf{G}_{2}^{n+c}
\end{align}
for $c<0$, where
\begin{align*}
& \textbf{B}^{rk}=[B^{rk,1},\ldots,B^{rk,s}]^T, \\
& \textbf{G}_{2}^{n+c}=[g_{2}(t^{n}+c_{1}\Delta t),\ldots,g_{2}(t^{n}+c_{s}\Delta t)]^T.
\end{align*}

The similar idea is used when dealing with a Neumann boundary condition. 

In our numerical tests, we will use $RK(2,3)$ and $RK(4,4)$ schemes to obtain third order accuracy and fourth order accuracy in time, respectively. Corresponding coefficients are listed as appendix.

\subsection{Positivity-preserving limiter}

The exact solution of \eqref{eq:1dadv} satisfies the positivity preserving principle, meaning that if the initial condition $u(x,0)\geq0$, then the exact solution $u(x,t)\geq0$ for any time $t>0$. In practice, it is highly desirable to have numerical schemes also satisfy such a property on the discrete level. It is even more crucial  for the Vlasov simulation, since negative values may trigger some nonphysical precess in plasmas \cite{qiu2011positivity}. Recently, Zhang {\em el at.} developed a high order positivity-preserving limiters for finite volume WENO methods and finite element DG methods, which is able to maintain high order accuracy of the original scheme and easy to implement \cite{zhang2010maximum,zhang2010positivity,zhang2011maximum,zhang2012maximum}. Later, Xu {\em et al.} \cite{xu2014parametrized,liang2014parametrized,xiong2013parametrized,xiong2016parametrized, xiong2014high} developed a parameter maximum principle preserving flux limiter for finite difference WENO schemes by limiting the high order flux towards a first order monotone flux. However, both limiters are exclusively designed for MOL type methods and hence cannot be directly applied in the MOL$^T$ setting. Below, we will formulate a new positivity-preserving (PP) limiter suited for the proposed WENO MOL$^T$ scheme, and also show that such a limiter is able to preserve positivity while maintaining high order accuracy of original schemes. 


 
Assume that we have $u^{n}_{i}\geq0$ for all $i$ at time $t^n$. After obtaining the numerical solutions $u^{n+1}_{i}$, we can rewrite our scheme in a conservative form  
$$u^{n+1}_{i}=u^{n}_{i}-\Delta t/\Delta x (\hat{f}_{i+1/2}-\hat{f}_{i-1/2}),$$
in which the artificial numerical fluxes $\hat{f}_{i+1/2}$ are recursively defined by
\begin{align*}
\hat{f}_{i+1/2}=\left\{\begin{array}{ll}
0, & i = -1,\\
\hat{f}_{i-1/2}-\Delta x/\Delta t(u^{n+1}_{i}-u^{n}_{i}), & i=0,\ldots,M.\\
\end{array}
\right.
\end{align*}

If we are able to modify the numerical flux $\hat{f}_{i+1/2}$ into $\tilde{f}_{i+1/2}$, such that
\begin{align}
\label{eq:pplimiter}
u^{new}_{i}=u^{n}_{i}-\Delta t/\Delta x (\tilde{f}_{i+1/2}-\tilde{f}_{i-1/2})\geq0, \ \ i=0,\ldots,M,
\end{align}
then the modified solution $u^{new}$ at time level $t=t^{n+1}$ will be non-negative automatically. Roughly speaking, the main idea of the limiter is to enforce the negative solution value back to zero by decreasing the outflow flux. For instance, when $c>0$, we will reset the numerical flux $\hat{f}_{i+1/2}$ if $u^{n+1}_{i}<0$. Details of the limiter are shown below. 

Firstly, we consider the case $c>0$ and a Dirichlet boundary condition. Numerical flux $\hat{f}_{i+1/2}$  is modified into $\tilde{f}_{i+1/2}$, starting from $i=1$ to $i=M$,
\begin{align}
\label{eq:limit}
\tilde{f}_{i+1/2}=\left\{\begin{array}{ll}
\tilde{f}_{i-1/2}+ \Delta x/\Delta t u^{n}_{i}, & \text{if}  \ u^{n+1,1}_{i}<0, \\
\hat{f}_{i+1/2}, & \text{otherwise,}\\ 
\end{array}
\right.
\end{align}
where
$$u_{i}^{n+1,1}=u^{n}_{i}-\Delta t/\Delta x (\hat{f}_{i+1/2}-\tilde{f}_{i-1/2}).$$
$\tilde{f}_{-1/2}=\hat{f}_{-1/2}$ and $\tilde{f}_{1/2}=\hat{f}_{1/2}$, due to the Dirichlet boundary condition. For a Nuemann boundary condition, we can also use \eqref{eq:limit} to modify fluxes. Once the modified fluxes are obtained, the positivity-preserving solution is computed by \eqref{eq:pplimiter}.


For periodic boundary conditions, however, we need an additional step in order to preserve the positivity and periodicity of the solution. In particular, we first modify  the numerical flux $\hat{f}_{i+1/2}$ into $\hat{\hat{f}}_{i+1/2}$ by \eqref{eq:limit} i.e., starting from $i=0$ into $i=M-1$, with
\begin{align*}
\hat{\hat{f}}_{i+1/2}=\left\{\begin{array}{ll}
\hat{f}_{i-1/2}+\Delta x/\Delta t u^{n}_{i}, & if \ u^{n+1,1}_{i}<0,\\
\hat{f}_{i+1/2}, & \text{otherwise},\\ 
\end{array}
\right.
\end{align*}
where
$$u_{i}^{n+1,1}=u^{n}_{i}-\Delta t/\Delta x (\hat{f}_{i+1/2}-\hat{\hat{f}}_{i-1/2}).$$
For periodicity, we further set $\tilde{f}_{-1/2}=\hat{\hat{f}}_{M-1/2}$. Note that since the flux at $x_{-1/2}$ is modified, the solution at $x_{0}$ may become negative. Hence, we need screen the solution one more time by the following procedure. Starting $i=0$, we compute
$$u_{i}^{n+1,2}=u^{n}_{i}-\Delta t/\Delta x (\hat{\hat{f}}_{i+1/2}-\tilde{f}_{i-1/2}).$$
If $u_{i}^{n+1,2}<0,$   we let 
$$\tilde{f}_{i+1/2}=\tilde{f}_{i-1/2}+\Delta x/\Delta t u^{n}_{i}.$$
Otherwise, let $i_0=i$ and for any $j$ with $i_0\leq j\leq M-1$, let 
$\tilde{f}_{j+1/2}=\hat{\hat{f}}_{j+1/2}.$ Finally, we are able to obtain the positivity-preserving solution $u^{new}$ via \eqref{eq:pplimiter}. Note that $i_0$ must be less than $M-1$ and hence $\tilde{f}_{M-1/2}=\tilde{f}_{-1/2}$. 


 
% the limiter \eqref{eq:limit} one more time to maintain mass conservation and periodic:
%\begin{enumerate}
%	\item Modify the numerical flux $\hat{f}_{i+1/2}$ into $\hat{\hat{f}}_{i+1/2}$, starting from $i=0$ into $i=M-1$, with
%	\begin{align*}
%	\hat{\hat{f}}_{i+1/2}=\left\{\begin{array}{ll}
%	\hat{f}_{i-1/2}+\Delta x/\Delta t u^{n}_{i}, & if \ u^{n+1,1}_{i}<0\\
%	\hat{f}_{i+1/2}, & \text{otherwise},\\ 
%	\end{array}
%	\right.
%	\end{align*}
%	where
%	$$u_{i}^{n+1,1}=u^{n}_{i}-\Delta t/\Delta x (\hat{f}_{i+1/2}-\hat{\hat{f}}_{i-1/2}),$$
%	
%	
%	\item Take $\tilde{f}_{-1/2}=\hat{\hat{f}}_{M-1/2}$. Then, modify the numerical flux $\hat{\hat{f}}_{i+1/2}$ into $\tilde{f}_{i+1/2}$, starting from $i=0$ into $i=M-1$, with
%	\begin{align*}
%	\tilde{f}_{i+1/2}=\left\{\begin{array}{ll}
%	\tilde{f}_{i-1/2}+\Delta x/\Delta t u^{n}_{i}, & if \ u^{n+1,2}_{i}<0\\
%	\hat{\hat{f}}_{i+1/2}, & \text{otherwise},\\ 
%	\end{array}
%	\right.
%	\end{align*}
%	where
%	$$u_{i}^{n+1,2}=u^{n}_{i}-\Delta t/\Delta x (\hat{\hat{f}}_{i+1/2}-\tilde{f}_{i-1/2}),$$
%	We can prove that $\tilde{f}_{M-1/2}=\tilde{f}_{-1/2}$. And define $\tilde{f}_{M+1/2}=\tilde{f}_{1/2}$ due to the periodic boundary conditions.
%\end{enumerate}


%For periodic boundary conditions,  we need to repeat the limiter \eqref{eq:limit} one more time to maintain mass conservation and periodic:
%\begin{enumerate}
%\item Modify the numerical flux $\hat{f}_{i+1/2}$ into $\hat{\hat{f}}_{i+1/2}$, starting from $i=0$ into $i=M-1$, with
%\begin{align*}
%\hat{\hat{f}}_{i+1/2}=\left\{\begin{array}{ll}
%\hat{f}_{i-1/2}+\Delta x/\Delta t u^{n}_{i}, & if \ u^{n+1,1}_{i}<0\\
%\hat{f}_{i+1/2}, & \text{otherwise},\\ 
%\end{array}
%\right.
%\end{align*}
%where
%$$u_{i}^{n+1,1}=u^{n}_{i}-\Delta t/\Delta x (\hat{f}_{i+1/2}-\hat{\hat{f}}_{i-1/2}),$$
%
%
%\item Take $\tilde{f}_{-1/2}=\hat{\hat{f}}_{M-1/2}$. Then, modify the numerical flux $\hat{\hat{f}}_{i+1/2}$ into $\tilde{f}_{i+1/2}$, starting from $i=0$ into $i=M-1$, with
%\begin{align*}
%\tilde{f}_{i+1/2}=\left\{\begin{array}{ll}
%\tilde{f}_{i-1/2}+\Delta x/\Delta t u^{n}_{i}, & if \ u^{n+1,2}_{i}<0\\
%\hat{\hat{f}}_{i+1/2}, & \text{otherwise},\\ 
%\end{array}
%\right.
%\end{align*}
%where
%$$u_{i}^{n+1,2}=u^{n}_{i}-\Delta t/\Delta x (\hat{\hat{f}}_{i+1/2}-\tilde{f}_{i-1/2}),$$
%We can prove that $\tilde{f}_{M-1/2}=\tilde{f}_{-1/2}$. And define $\tilde{f}_{M+1/2}=\tilde{f}_{1/2}$ due to the periodic boundary conditions.
%\end{enumerate}
%
When $c<0$, wind blows from right to left, and we will reset the numerical flux $\hat{f}_{i-1/2}$ if $u^{n+1}_{i}<0$. The similar idea can be used for different boundary conditions. 

Below, we show that the PP-limiter can preserve positivity while maintaining the previous high order. In particular, we have the following proposition.

\begin{prop} Consider the WENO MOL$^T$scheme is used for solving \eqref{eq:1dadv} and assume that the numerical solution $u^{n+1}_{i}$ is $p$-th order accurate in space and $q$-th order accurate in time, i.e., the global error
	$$e_i^{n+1} = |u_i^{n+1}-u(x_i,t^{n+1})|=\mathcal{O}(\Delta x^p+\Delta t^q),\quad \forall i,$$
	where $u(x_{i},t^{n+1})$ is the exact solution. If  the  proposed PP-limiter \eqref{eq:pplimiter} with \eqref{eq:limit} is applied, then 
		$$\tilde{e}_i^{n+1} = |u_i^{new}-u(x_i,t^{n+1})|=\mathcal{O}(\Delta x^{p-1}+\Delta x^{-1}\Delta t^q),\quad \forall i$$
		for the worst case, when $\Delta t=\mathcal{O}(\Delta x)$. 
\end{prop}

{\bf Proof.} Without loss of generality, we only consider \eqref{eq:1dadv} with $c>0$ and a Dirichlet boundary condition is imposed for brevity. Let $u^{n+1}_i$ be the first solution value that is less than zero starting from $u^{n+1}_{1}$, i.e., $u^{n+1}_i<0$ and  $u^{n+1}_j\ge0,\,1\le j<i.$ Then we have $\tilde{f}_{j-1/2}=\hat{f}_{j-1/2},\, 0\le j\le i,$ and $\tilde{f}_{i+1/2} = \tilde{f}_{i-1/2}+ \Delta x/\Delta t u^{n}_{i},$
such that $u^{new}_i=0.$ Recalling that $u(x_i,t^{n+1})\ge 0$ and $e_i^{n+1}=\mathcal{O}(\Delta x^p+\Delta t^q),$ and hence $\tilde{e}_i^{n+1}=\mathcal{O}(\Delta x^p+\Delta t^q).$ Also note that the modification of flux 
$$\tilde{f}_{i+1/2}-\hat{f}_{i+1/2} =\Delta x/\Delta t u^{n+1}_{i}=\mathcal{O}(\Delta x^{p}+\Delta t^{q})$$ 
is a negative high order quantity.

Now, we consider the effect of the modification of flux $\tilde{f}_{i+1/2}$ to the next point value in terms of accuracy. First, we need to compute $$u_{i+1}^{n+1,1}=u^{n}_{i+1}-\Delta t/\Delta x (\hat{f}_{i+3/2}-\tilde{f}_{i+1/2}).$$ Several cases need to be taken into account.

\noindent{\bf Case (1)} If $u_{i+1}^{n+1,1}\ge0.$ Then, $\tilde{f}_{i+3/2}=\hat{f}_{i+3/2}$ by \eqref{eq:limit}, and $u^{new}_{i+1}=u_{i+1}^{n+1,1}.$ We have
%
$$|u^{new}_{i+1}-u^{n+1}_{i+1}|=|\Delta t/\Delta x (\tilde{f}_{i+1/2}-\hat{f}_{i+1/2})|=\mathcal{O}(\Delta x^{p}+\Delta t^{q}).$$
Hence, $$\tilde{e}_{j+1}^{n+1}=|u^{new}_{i+1}-u(x_{i+1},t^{n+1})|\leq |u^{new}_{i+1}-u^{n+1}_{i+1}|+e_{i+1}^{n+1}=\mathcal{O}(\Delta x^{p}+\Delta t^{q}).$$ 

\noindent{\bf Case (2)}
If $u_{i+1}^{n+1,1}<0.$ Then, $\tilde{f}_{i+3/2}=\tilde{f}_{i+1/2}+ \Delta x/\Delta t u^{n}_{i+1}$ by \eqref{eq:limit}, and $u^{new}_{i+1}=0$. There are two cases we need to treat differently. If $u_{i+1}^{n+1}<0$, then by the same argument we used to treat the case at $x_{i}$, we have  $u^{n+1}_{i+1}=\mathcal{O}(\Delta x^{p}+\Delta t^{q})$  and hence $e^{n+1}_{i+1}=\mathcal{O}(\Delta x^{p}+\Delta t^{q})$. If $u_{i+1}^{n+1}\ge0$, then we have 
$$|u_{i+1}^{n+1,1}-u_{i+1}^{n+1}|=|\Delta t/\Delta x(\tilde{f}_{i+1/2}-\hat{f}_{i+1/2})|=\mathcal{O}(\Delta x^{p}+\Delta t^{q}).$$ 
Further, since  $u_{i+1}^{n+1,1}<0$ and  $u_{i+1}^{n+1}>0$, combining the above estimate, we have
$$|u^{n+1}_{i+1}|=\mathcal{O}(\Delta x^{p}+\Delta t^{q}).$$
Consequently,   $$\tilde{e}_{j+1}^{n+1}=|u^{new}_{i+1}-u(x_{i+1},t^{n+1})|=|u(x_{i+1},t^{n+1})|\leq |u^{n+1}_{i+1}|+e_{j+1}^{n+1}=\mathcal{O}(\Delta x^{p}+\Delta t^{q}).$$
%
We also have the following modification of the flux
\begin{equation}\label{eq:modi2}
	\tilde{f}_{i+3/2}-\hat{f}_{i+3/2} =\Delta x/\Delta t u^{n+1}_{i} + \tilde{f}_{i+1/2}-\hat{f}_{i+1/2} = \Delta x/\Delta t (u^{n+1}_{i+1} + u^{n+1}_{i})=\mathcal{O}(\Delta x^{p}+\Delta t^{q}).
\end{equation}
	

For both cases, we have shown that $\tilde{e}_{j+1}^{n+1}=\mathcal{O}(\Delta x^{p}+\Delta t^{q}),$ i.e., the PP-limiter preserves the order of accuracy.  Moreover, for case (1)
since the flux $\hat{f}_{i+3/2}$ is not changed, we can move on to consider the solution value at $x_{i+2}$ with the same procedure as the case at $x_{i}$. The situation of case (2) is more complicated when considering the subsequent effect of the modification of flux \eqref{eq:modi2}. Again, we need to consider two cases.

\noindent{\bf Case (2.1)} If $u_{i+2}^{n+1,1}\ge0.$ Similar to case (1) above, the flux at $\tilde{f}_{i+5/2}$ should remain the same, i.e., $\tilde{f}_{i+5/2}=\hat{f}_{i+5/2}$. By \eqref{eq:modi2}
$$|u^{new}_{i+2}-u^{n+1}_{i+2}|=|\Delta t/\Delta x (\tilde{f}_{i+3/2}-\hat{f}_{i+3/2})|=\mathcal{O}(\Delta x^{p}+\Delta t^{q}),$$
and consequently, $$\tilde{e}_{i+2}^{n+1}=\mathcal{O}(\Delta x^{p}+\Delta t^{q}).$$

\noindent{\bf Case (2.2)} If $u_{i+2}^{n+1,1}<0$. We can repeat the analysis of case (2) and obtain that 
$$|u^{n+1}_{i+2}|=\mathcal{O}(\Delta x^{p}+\Delta t^{q}),$$
which gives the estimate
$$\tilde{e}_{i+2}^{n+1}=\mathcal{O}(\Delta x^{p}+\Delta t^{q}),$$ and the modification of the flux
\begin{equation}\label{eq:modi3}
\tilde{f}_{i+5/2}-\hat{f}_{i+5/2} = \Delta x/\Delta t (u^{n+1}_{i+2}+u^{n+1}_{i+1} + u^{n+1}_{i})=\mathcal{O}(\Delta x^{p}+\Delta t^{q}).
\end{equation}

More generally, assume that the fluxes are successively modified with at most constant many times, i.e., there exists a constant $K_0$ independent of $\Delta x$ and $\Delta t$, such that if the fluxes $\tilde{f}_{i+k+1/2}$ for $0\le k\le K$ are successively changed based on
$$\tilde{f}_{i+k+1/2} = \hat{f}_{i+k+1/2} +\Delta x/\Delta t \sum_{l=0}^ku^{n+1}_{i+l},$$
then $K$ is always bounded by $K_0$. We have $$\tilde{e}^{n+1}_i=\mathcal{O}(\Delta x^{p}+\Delta t^{q}).$$ For the worst cases, the fluxes may be successively modified with $\mathcal{O}(1/\Delta x)$ times, then the accumulation of error leads to one order reduction in space, i.e., 
$$\tilde{e}^{n+1}_i=\mathcal{O}(\Delta x^{p-1}+\Delta x^{-1}\Delta t^{q}).$$

\begin{rem}
	In our simulations, the worst cases never happened: $K_0$ is always a constant independent of mesh sizes, and optimal accuracy is observed for all our accuracy tests.
\end{rem}
